The Cosmic Hunt for Members in the Outskirts of Ultra Faint Dwarf Galaxies: Ursa Major I, Coma Berenices, and Bo\"otes I

Gaia EDR3 data was used to identify potential members in the outskirts of three ultra faint dwarf (UFD) galaxies; Coma Berenices (> 2Rh), Ursa Major I ($\sim$ 4Rh), and Bo\"otes I ($\sim$ 4Rh), as well as a new member in the central region of Ursa Major I. These targets were observed with the Gemini GRACES spectrograph, which was used to determine precision radial velocities and metallicities that confirm their associations with the UFD galaxies. The spectra were also used to measure absorption lines for 10 elements (Na, Mg, K, Ca, Sc, Ti, Cr, Fe, Ni, and Ba), which confirm that the chemical abundances of the outermost stars are in good agreement with stars in the central regions. The abundance ratios and chemical patterns of the stars in Coma Berenices are consistent with contributions from SN Ia, which is unusual for its star formation history and in conflict with previous suggestions that this system evolved chemically from a single core collapse supernova event. The chemistries for all three galaxies are consistent with the outermost stars forming in the central regions, then moving to their current locations through tidal stripping and/or supernova feedback. In Bo\"otes I, however, the lower metallicity and lack of strong carbon enrichment of its outermost stars could also be evidence of a dwarf galaxy merger.

==> extratables.tex <==

\begin{table}
\caption{Mean and standard deviation of the 1D LTE line scatter for species for the EW and synthesis results for each star. Number of lines in parentheses.}
\begin{tabular}{lrrrrrrrrrr}
              &       \multicolumn{2}{c}{CB-1 }             &       \multicolumn{2}{c}{CB-2 }             & \multicolumn{2}{c}{UMaI-1 }                 & \multicolumn{2}{c}{UMaI-2 }                 & \multicolumn{2}{c}{BooI-2 }                  \\
                      \cmidrule(lr){2-3}                            \cmidrule(lr){4-5}                      \cmidrule(lr){6-7}                            \cmidrule(lr){8-9}                            \cmidrule(lr){10-11}
{}            &    log(X/H)$_{EW}$   &  log(X/H)$_{syn}$    &    log(X/H)$_{EW}$   &    log(X/H)$_{syn}$  &  log(X/H)$_{EW}$     &    log(X/H)$_{syn}$  &   log(X/H)$_{EW}$    &    log(X/H)$_{syn}$  &  log(X/H)$_{EW}$      &    log(X/H)$_{syn}$  \\
\midrule
\textbf{26.0} &  4.62$\pm$0.20  (73) &  4.59$\pm$0.20  (69) &  5.35$\pm$0.22  (41) &  5.28$\pm$0.22  (38) &  4.99$\pm$0.18  (42) &  4.97$\pm$0.22  (41) &  5.08$\pm$0.27  (43) &  5.14$\pm$0.29  (43) &   5.01$\pm$0.20  (55) &  4.94$\pm$0.21  (56) \\
\textbf{26.1} &  4.53$\pm$0.20 ~~(4) &  4.56$\pm$0.20 ~~(4) &  5.18$\pm$0.29 ~~(5) &  5.29$\pm$0.26 ~~(5) &  5.46$\pm$0.18 ~~(2) &  5.53$\pm$0.22 ~~(2) &  5.04$\pm$0.27 ~~(2) &  5.08$\pm$0.29 ~~(2) &   5.05$\pm$0.24 ~~(6) &  5.02$\pm$0.21 ~~(6) \\
\textbf{11.0} &  3.66$\pm$0.20 ~~(2) &  3.40$\pm$0.20 ~~(2) &  3.94$\pm$0.22 ~~(2) &  3.77$\pm$0.22 ~~(2) &  3.45$\pm$0.18 ~~(2) &  3.39$\pm$0.22 ~~(2) &  3.09$\pm$0.27 ~~(2) &  3.00$\pm$0.29 ~~(2) &   3.12$\pm$0.20 ~~(2) &  2.89$\pm$0.21 ~~(2) \\
\textbf{12.0} &  5.59$\pm$0.20 ~~(3) &  5.45$\pm$0.20 ~~(3) &  5.45$\pm$0.22 ~~(3) &  5.53$\pm$0.22 ~~(3) &  5.30$\pm$0.18 ~~(3) &  5.55$\pm$0.22 ~~(1) &  5.62$\pm$0.27 ~~(1) &  5.19$\pm$0.29 ~~(3) &   5.80$\pm$0.20 ~~(1) &  5.60$\pm$0.21 ~~(1) \\
\textbf{19.0} &  2.80$\pm$0.20 ~~(1) &                  (0) &                  (0) & <2.43$\pm$0.20 ~~(0) &  3.09$\pm$0.20 ~~(1) &                  (0) &  2.87$\pm$0.20 ~~(1) &                ~~(0) &   3.18$\pm$0.21 ~~(1) &                  (0) \\
\textbf{20.0} &  4.20$\pm$0.11  (13) &  4.06$\pm$0.15  (13) &  3.96$\pm$0.38 ~~(5) &  3.80$\pm$0.31 ~~(5) &  3.94$\pm$0.31  (11) &  3.92$\pm$0.34  (10) &  4.24$\pm$0.47 ~~(6) &  4.04$\pm$0.45 ~~(6) &   4.07$\pm$0.19  (12) &  4.02$\pm$0.21  (12) \\
\textbf{21.0} &                  (0) &      $\pm$0.20 ~~(1) &                  (0) &      $\pm$0.20 ~~(1) &                  (0) &      $\pm$0.20 ~~(0) &                  (0) &      $\pm$0.20 ~~(1) &                   (0) &      $\pm$0.20 ~~(1) \\
\textbf{22.0} &  2.29$\pm$0.11 ~~(7) &  2.32$\pm$0.12 ~~(7) &  3.03$\pm$0.27 ~~(5) &  3.15$\pm$0.22 ~~(3) &  2.88$\pm$0.18 ~~(2) &  2.80$\pm$0.22 ~~(2) &                  (0) &                  (0) &   2.86$\pm$0.20 ~~(4) &  2.88$\pm$0.21 ~~(4) \\
\textbf{22.1} &  2.45$\pm$0.20 ~~(4) &  2.42$\pm$0.20 ~~(4) &                  (0) &                  (0) &  3.36$\pm$0.18 ~~(3) &  3.22$\pm$0.22 ~~(3) &                  (0) &                  (0) &   2.66$\pm$0.20 ~~(2) &  2.58$\pm$0.21 ~~(2) \\
\textbf{24.0} &  2.58$\pm$0.20 ~~(3) &  2.48$\pm$0.20 ~~(3) &  3.48$\pm$0.22 ~~(3) &  3.38$\pm$0.22 ~~(3) &  2.59$\pm$0.18 ~~(2) &  2.74$\pm$0.22 ~~(2) &  3.25$\pm$0.27 ~~(2) &  3.35$\pm$0.29 ~~(2) &   2.57$\pm$0.20 ~~(2) &  2.74$\pm$0.21 ~~(2) \\
\textbf{28.0} &  3.21$\pm$0.20 ~~(2) &  3.12$\pm$0.20 ~~(2) &  4.58$\pm$0.20 ~~(5) &  4.61$\pm$0.18 ~~(5) &  3.80$\pm$0.18 ~~(4) &  3.79$\pm$0.22 ~~(4) &  3.79$\pm$0.27 ~~(2) &  3.68$\pm$0.29 ~~(2) &   3.61$\pm$0.16 ~~(5) &  3.57$\pm$0.22 ~~(5) \\
\textbf{56.1} & -1.75$\pm$0.20 ~~(2) &   -1.82$\pm$0.2  (2) & -0.81$\pm$0.22 ~~(2) & -0.91$\pm$0.22 ~~(2) & -0.62$\pm$0.18 ~~(3) & -0.62$\pm$0.22 ~~(3) & -0.50$\pm$0.27 ~~(3) & -0.54$\pm$0.29 ~~(3) &  -1.46$\pm$0.20 ~~(2) & -1.52$\pm$0.21 ~~(2) \\
\bottomrule
\end{tabular}
\label{tab:synVSew}
\end{table}

\begin{table}
\caption{Hyperfine structure corrections for Ba. }
\begin{tabular}{llllll}
\toprule
{} &  CB-1 &   CB-2 &  UMaI-1 &  UMaI-2 & BooI-2 \\
\midrule
\textbf{5853.7} &      &       &     0 & -0.21 &       \\
\textbf{6141.7} & -0.1 & -0.12 &  -0.1 & -0.23 &  -0.1 \\
\textbf{6496.9} &    0 & -0.14 & -0.05 & -0.06 &     0 \\
\midrule
\textbf{mean}   &-0.05 & -0.13 &-0.08 & -0.17 & -0.05 \\
\bottomrule
\end{tabular}
\label{tab:hyperfine}
\end{table}



\begin{table}
\caption{Mean and standard deviation for NLTE corrections from two databases, Inspect and MPIA. K and Ba corrections are from \citet{Andrievsky10} and Mashonkina database respectively, and marked in the Inspect column with a *. (n) is the number of lines in that species for which corrections were available. Inspect takes in the EW when calculating the correction, MPIA does not. MPIA has ~2x as many lines in our sample as Inspect does. MPIA gives larger corrections, or in a small number of cases, the same.}
\begin{tabular}{lrrrrrrrrrrrrrrr}
              &              \multicolumn{2}{c}{CB-1 }      &       \multicolumn{2}{c}{CB-2 }             & \multicolumn{2}{c}{UMaI-1 }                & \multicolumn{2}{c}{UMaI-2 }                 & \multicolumn{2}{c}{BooI-2 }  \\
                             \cmidrule(lr){2-3}                     \cmidrule(lr){4-5}                      \cmidrule(lr){6-7}                           \cmidrule(lr){8-9}                            \cmidrule(lr){10-11}
{species}     &        Inspect (n)   &           MPIA (n)   &       Inspect (n)    &       MPIA (n)       &     Inspect (n)     &      MPIA (n)        &         Inspect (n)  &      MPIA (n)        &     Inspect (n)       &      MPIA (n)         \\
\midrule
\textbf{26.0} &  0.11$\pm$0.02  (16) &  0.20$\pm$0.02  (34) &  0.15$\pm$0.05  (10) &  0.16$\pm$0.03  (24) &   0.1$\pm$0.03 (12) &  0.12$\pm$0.04  (22) &  0.14$\pm$0.03  (12) &  0.16$\pm$0.03  (24) &   0.10$\pm$0.04  (13) &  0.15$\pm$0.03  (30)  \\
\textbf{26.1} & -0.06$\pm$0.07 ~~(3) &  0.09$\pm$0.00 ~~(1) & -0.01$\pm$0.02 ~~(4) &  0.04$\pm$0.03 ~~(2) &  -0.01$\pm$0.00 (1) &  0.00$\pm$0.00 ~~(1) & -0.03$\pm$0.02 ~~(3) &  0.08$\pm$0.00 ~~(1) &  -0.03$\pm$0.02 ~~(5) &  0.05$\pm$0.04 ~~(2)  \\
\textbf{11.0} & -0.28$\pm$0.01 ~~(2) &                      & -0.47$\pm$0.02 ~~(2) &                      &  -0.11$\pm$0.02 (2) &                      & -0.24$\pm$0.03 ~~(2) &                      &  -0.20$\pm$0.01 ~~(2) &                       \\
\textbf{12.0} & -0.02$\pm$0.03 ~~(3) &  0.08$\pm$0.02 ~~(3) & -0.02$\pm$0.02 ~~(3) &  0.06$\pm$0.02 ~~(3) &                     &  0.05$\pm$0.03 ~~(3) &                      &  0.06$\pm$0.01 ~~(3) &  -0.08$\pm$0.00 ~~(1) &  0.06$\pm$0.00 ~~(1)  \\
\textbf{19.0} & *0.21$\pm$0.05 ~~(1) &                      & *0.33$\pm$0.05 ~~(1) &                      &  *0.21$\pm$0.05 (1) &                      & *0.21$\pm$0.05 ~~(1) &                      &  *0.21$\pm$0.05 ~~(1) &                       \\
\textbf{20.0} &                      &  0.19$\pm$0.05 ~~(7) &                      &  0.15$\pm$0.02 ~~(3) &                     &  0.13$\pm$0.06 ~~(7) &                      &  0.20$\pm$0.04 ~~(6) &                       &  0.16$\pm$0.05 ~~(7)  \\
\textbf{21.0} &                      &                      &                      &                      &                     &                      &                      &                      &                       &                       \\
\textbf{22.0} &  0.34$\pm$0.03 ~~(3) &  0.47$\pm$0.04 ~~(6) &  0.14$\pm$0.01 ~~(2) &  0.47$\pm$0.11 ~~(4) &   0.20$\pm$0.00 (1) &  0.47$\pm$0.10 ~~(2) &                      &                      &   0.24$\pm$0.04 ~~(3) &  0.40$\pm$0.04 ~~(3)  \\
\textbf{22.1} &                      &  0.08$\pm$0.02 ~~(4) &                      & -0.08$\pm$0.00 ~~(1) &                     & -0.05$\pm$0.06 ~~(3) &                      &                      &                       &  0.07$\pm$0.02 ~~(2)  \\
\textbf{24.0} &                      &  0.45$\pm$0.05 ~~(3) &                      &  0.37$\pm$0.05 ~~(3) &                     &  0.33$\pm$0.02 ~~(2) &                      &  0.41$\pm$0.00 ~~(2) &                       &  0.39$\pm$0.00 ~~(2)  \\
\textbf{28.0} &                      &                      &                      &                      &                     &                      &                      &                      &                       &                       \\
\textbf{56.1} & *0.09$\pm$0.02 ~~(1) &                      & *0.04$\pm$0.02 ~~(1) &                      &  *0.09$\pm$0.02 (1) &                      & *0.05$\pm$0.02 ~~(1) &                      &  *0.09$\pm$0.02 ~~(1) &                       \\ 
\bottomrule
\end{tabular}
\label{tab:nltesummary}
\end{table}









% \begin{figure}
% 	\includegraphics[width=10cm]{figs/abun_diff.2.jpg}
%     \caption{abundance differences in individual iron lines for CB1 between synth and EW}
%     \label{fig:diff}
% \end{figure}

% \begin{figure}
% 	\includegraphics[width=\columnwidth]{figs/FeHvsR_h.png}
%     \caption{metallicity vs half-light radius. Our data LTE as squares, NLTE as stars, all literature data as dots.  \kv{Add RV vs RH beside this.  Add errorbars, if possible.  Check points similar to earlier figures.  Then drop it into Section 7.1.}  
%     \label{fig:rh}  }
% \end{figure}



==> tables/1.observations.tex <==
\begin{table*}
\caption{Gaia EDR3 data for each target, as well as our GRACES observational details and their locations in each UFD. In the absence of consistent naming conventions for UFD stars, we use the following naming scheme in this paper, and include Gaia source IDs for cross-matching purposes.  }
\label{tab:obs}
\begin{tabular}{lllccccccccl}
\toprule
 Name  &     RA J2000 &   Dec J2000 & Obs Date   &    G & BP$-$RP & t$_{\rm exp}$ & N$_{\rm exp}$ & SNR  & loc.  & A$_{\rm V}$ & Gaia sourceID \\
 & (hh\,mm\,ss) & (dd\,mm\,ss) & & (mag) & (mag) & (sec) & & (5200, 6000) & (R$_{\rm h}$) & \\
\midrule
CB-1   & 12 26 43.5 & 24 04 45.7 & 2021-01-07 & 15.40 & 1.42 & 900 & 3 & 20, 35 & 2.5 & 0.054 & 3959888486031303424 \\
CB-2   & 12 26 03.9 & 24 00 26.1 & 2021-01-07 & 16.85 & 1.14 & 1800 & 2 & 10, 16 & 2.5 & 0.061 & 3959884740819808256 \\
BooI-2 & 14 01 32.6 & 15 06 50.7 & 2021-05-08 & 16.52 & 1.41 & 2400 & 4 & 15, 30 & 4.0 & 0.058 & 1231264907837100800 \\
UMaI-1 & 10 32 30.1 & 51 57 04.9 & 2021-01-08 & 17.12 & 1.48 & 1800 & 3 & 7, 15 & 3.7 & 0.049 & 847716356845689216 \\
UMaI-2 & 10 35 28.9 & 51 57 01.5 & 2021-01-08 & 17.82 & 1.31 & 2400 & 4 & 7, 15 & 0.7 & 0.052 & 849020961751785472 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/2.gal_par.tex <==
\tabcolsep=0.17cm
\begin{table}
\caption[]{Galactic parameters for our three UFD galaxies from \citet[][updated 2021\footnotemark]{McConnachie2012} %\kv{You mentioned UMa I is close to pericentre now in the text in Section 7 - is there a reference if that is no longer true - can we write this such that we are not waiting on Asya's next paper?}.  
RV is the range in radial velocities, D$_\odot$ is the heliocentric distance, {\sl ell} and $\phi$ are the ellipticity and position angle of the isophotes, and R$_{\rm h}$ is the half light radius, for each UFD. }
\begin{tabular}{lrccccc}
\toprule
 Name   & RV range              & D$_\odot$ & ell   & $\phi$      & R$_{\rm h}$ & R$_{\rm h}$\\
        &  (\kms)               & (kpc)     &       & (deg)       & (arcmin) & (pc)\\
\midrule
Com~Ber  &    97.2 to \,\, 99.0 & 40 $\pm$4 & 0.37  &    $-$58    & \ 5.63  &  65 \\
UMa~I    & $-$56.7 to   $-$53.9 & 97 $\pm$4 & 0.57  &   \ \ 67    & \ 8.34  & 235 \\
Boo~I    &    96.9 to     101.1 & 66 $\pm$2 & 0.25  &  \ \ \ 7    &  11.26  & 217 \\ 
\bottomrule
\end{tabular}
\label{tab:galpar}
\end{table}


==> tables/3.stel_par.tex <==
\begin{table}
\caption{The stellar parameters, effective temperature (\teff) and surface gravity (\logg) for our \textsc{MARCS} model atmospheres.  Metallicities ([Fe/H]$_{\rm LTE}$) are from our spectral line analysis (see Section~\ref{sec:spectra}), and microturbulence ($\xi$) is calculated from \citet{Mashonkina17}. Values of \logg$<$0.5 were set to 0.5 to avoid extrapolating outside the \textsc{MARCS} grid.  Radial velocities (RV) are found with \textsc{IRAF}/{\sl fxcor} from our spectra. Parameters for HD122563 are from \citet{Mashonkina17} and \citet{Karicova2020}. 
%
% BooI stars all seem to go by Boo-980 for instance. Vargas refers to UMaI stars as UMaI-S2. Com\,Ber stars are referred to by Frebel as Comber-S1 etc. 
}
\tabcolsep=0.08cm
\begin{tabular}{lccccc}
\toprule
Name  & \teff  & \logg  & $\xi$  & [Fe/H]$_{\rm LTE}$ & RV  \\
   &  (K) &  (dex) & (\kms) & (dex) & (\kms) \\
\midrule
CB-1   & 4385 $\pm$81 & 0.33 $\pm$0.12 & 2.1$\pm$0.1  & $-2.88 \pm$0.15   & \,\, 91.76 $\pm$0.18 \\
CB-2   & 4879 $\pm$99 & 1.24 $\pm$0.12 & 2.5$\pm$0.1  & $-2.16 \pm$0.12   & \,\, 95.86 $\pm$0.27 \\
BooI-2 & 4390 $\pm$70 & 0.41 $\pm$0.08 & 2.3$\pm$0.1  & $-2.49 \pm$0.14   & \,\, 99.25 $\pm$1.09 \\ 
UMaI-1 & 4308 $\pm$68 & 0.28 $\pm$0.12 & 2.1$\pm$0.1  & $-2.50 \pm$0.12   & $-$51.73 $\pm$0.38 \\
UMaI-2 & 4574 $\pm$83 & 0.75 $\pm$0.11 & 2.4$\pm$0.1  & $-2.42 \pm$0.20   & $-$53.78 $\pm$0.98 \\
HD122563 & 4635 $\pm$34 & 1.40 $\pm$0.04 & 1.7~~~~~~~~ & $-2.75 \pm$0.12  & — \\
\bottomrule
\end{tabular}
\label{tab:param}
\end{table}

==> tables/4.linelist_abundances.tex <==

\tabcolsep=0.17cm

\begin{longtable}{llrrrrrrrrrrrrrrr}
\caption{Chemical abundances for each star using both measurement methods for every single line. n: line too noisy; w: line too weak; s: line too strong, EW $>150$ m$\Angstrom$; b: line part of a blend; italics: EW $>150$ m$\Angstrom$, but no other lines available, so they are kept.}
\label{tab:linelistfull}
\endfirsthead
\endhead
\hline
       &      & \multicolumn{3}{c}{CB-1 (SNR=20)}        & \multicolumn{3}{c}{CB-2 (SNR=10)}   & \multicolumn{3}{c}{UMaI-1 (SNR=7)}  & \multicolumn{3}{c}{UMaI-2 (SNR=7)}    &  \multicolumn{3}{c}{BooI-2 (SNR=15 )}   \\
 \cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(lr){9-11}\cmidrule(lr){12-14} \cmidrule(lr){15-17} 
 Wave. & Elem & EW   & X$_{\rm EW}$ & X$_{\rm SYN}$      & EW   & X$_{\rm EW}$ & X$_{\rm SYN}$ & EW   & X$_{\rm EW}$ & X$_{\rm SYN}$ & EW   & X$_{\rm EW}$ & X$_{\rm SYN}$   & EW   & X$_{\rm EW}$ & X$_{\rm SYN}$ \\

\hline\hline
   4871.318 &    26 &   60 &        4.1 &        4.2  &   n  &            &             &  n   &            &             &  n   &            &              & n    &            &             \\
   4872.138 &    26 &   80 &       4.74 &        4.85 &   w  &            &             &  n   &            &             &  n   &            &              & 115  &   5.13     &      5.50   \\
   4890.755 &    26 &   75 &       4.41 &         4.3 &   n  &            &             &  n   &            &             &  n   &            &              & 125  &   5.07     &      5.20   \\
   4891.492 &    26 &   95 &        4.5 &        4.45 &   n  &            &             &  n   &            &             &  n   &            &              & 110  &   4.53     &      4.88   \\
   4918.994 &    26 &   80 &       4.46 &         4.3 &  105 &       5.06 &        5.53 &  n   &            &             &  n   &            &              & 150  &   5.45     &      5.50   \\
   4920.502 &    26 &   85 &       4.07 &        4.5  &  140 &       5.23 &        5.1  &  n   &            &             &  n   &            &              & 150  &   4.97     &      4.92   \\
   4939.687 &    26 &  105 &       4.83 &        5.1  &  s/b &            &             &  n   &            &             &  n   &            &              & 135  &   5.11     &      4.82   \\
   4966.089 &    26 &   55 &       5.05 &        5.1  &   w  &            &             &  n   &            &             &  n   &            &              &  65  &   5.07     &      5.20   \\
   4994.130 &    26 &  105 &       4.61 &         4.8 &   90 &       5.08 &        5.58 &  n   &            &             &  n   &            &              & 150  &   5.13     &      5.10   \\
   5006.119 &    26 &   60 &       4.27 &         4.4 &   n  &            &             &  n   &            &             &  n   &            &              & 105  &   4.83     &      5.10   \\
   5012.068 &    26 &  135 &       4.64 &         4.4 &  113 &       5.00 &        4.8  &  n   &            &             &  n   &            &              &  s   &            &             \\
   5041.072 &    26 &  100 &        4.7 &         4.8 &   w  &            &             &  n   &            &             &  n   &            &              & 135  &   5.05     &      5.57   \\
   5041.756 &    26 &  100 &        4.6 &        4.8  &   n  &            &        4.9  &  n   &            &             &  n   &            &              &  s   &            &             \\
   5049.819 &    26 &   90 &       4.73 &         4.6 &   n  &            &             &  n   &            &             &  n   &            &              & 115  &   4.94     &      4.90   \\
   5051.635 &    26 &  130 &       4.78 &         4.7 &   s  &            &             &  n   &            &             &  n   &            &              & 135  &   4.64     &      4.90   \\
   5068.766 &    26 &   65 &       5.11 &           5 &   n  &            &             &  n   &            &             &  w   &            &              &  n   &            &             \\
   5110.413 &    26 &   s  &            &             &   s  &            &             &  s   &            &             &  135 &       4.66 &        4.4   &  n   &            &             \\
   5123.720 &    26 &  110 &       4.87 &             &   s  &            &             &  s   &            &             &  120 &       5.16 &        5.12  &  n   &            &             \\
   5127.360 &    26 &  100 &       4.77 &             &   s  &            &             &   s  &            &             &  130 &       5.36 &        5.32  &  n   &            &             \\
   5150.840 &    26 &   95 &       4.59 &             &   n  &            &             &  130 &       4.74 &        4.55 &  125 &       5.18 &        5.4   &  n   &            &             \\
   5151.911 &    26 &  100 &       4.97 &             &   n  &            &             &  115 &        4.8 &        4.75 &  w   &            &              &  n   &            &             \\
   5191.454 &    26 &   70 &        4.6 &         4.8 &   70 &       4.87 &        5.05 &  w   &            &             &  w   &            &              &  n   &            &             \\
   5192.344 &    26 &   55 &       4.17 &         4.4 &  120 &       5.47 &        5.95 &   n  &            &             &  w   &            &              &  n   &            &             \\
   5194.942 &    26 &  110 &       4.62 &         4.4 &  s/b &            &             &   n  &            &             &  n   &            &              &  n   &            &             \\
   5198.711 &    26 &   50 &       4.71 &         4.7 &   n  &            &             &  s   &            &             &  s   &            &              &  n   &            &             \\
   5216.274 &    26 &  125 &       4.98 &        4.75 &   s  &            &             &  n   &            &             &  140 &       5.27 &        5.60  &  n   &            &             \\
   5232.940 &    26 &  105 &       4.69 &        4.65 &  140 &       5.52 &        5.05 &  s   &            &             &  130 &       5.02 &        5.17  & 115  &   4.64     &      4.98   \\
   5247.050 &    26 &   45 &       4.48 &        4.8  &   n  &            &             &  130 &       5.08 &         5.4 &  105 &       5.55 &        5.40  &  80  &   4.79     &      4.95   \\
   5250.210 &    26 &   80 &       4.91 &         4.7 &   n  &            &             &  125 &       5.13 &        4.85 &   90 &       5.34 &        5.68  &  85  &   4.83     &      5.00   \\
   5250.646 &    26 &   60 &        4.9 &        4.75 &  90  &       5.78 &             &  n/b &            &             &  n   &            &              & 100  &   5.34     &      5.40   \\
   5254.956 &    26 &   80 &       4.75 &         4.8 &  s/b &            &             &  135 &       5.14 &         5.4 &  120 &       5.56 &        5.40  &  90  &   4.73     &      4.85   \\
   5266.555 &    26 &   80 &       4.63 &        4.55 &  105 &       5.28 &        5.35 &  n   &            &             &  105 &      4.99  &        5.25  & 115  &   5.01     &      4.82   \\
   5281.790 &    26 &   50 &       4.72 &        4.65 &   80 &       5.47 &        5.55 &  n   &            &             &   85 &       5.26 &        5.40  & 105  &   5.43     &      5.18   \\
   5283.621 &    26 &   65 &       4.66 &         4.5 &   70 &       4.99 &             &  110 &       5.07 &        5.2  &   n  &            &              &  85  &   4.82     &      4.80   \\
   5307.361 &    26 &   50 &       4.66 &        4.75 &   w  &            &             &  n   &            &             &  w   &            &              &  85  &   5.01     &      5.20   \\
   5324.179 &    26 &   70 &       4.36 &        4.35 &   n  &            &             &  s   &            &             &  120 &       5.11 &        5.2   & 140  &   5.31     &      5.03   \\
   5328.532 &    26 &  120 &       4.55 &         4.4 &   n  &            &             &  n   &            &             &  n   &            &              &  s   &            &             \\
   5332.900 &    26 &   60 &        4.6 &         4.75&  s/b &            &             &  125 &       5.17 &        5.5  &  100 &       5.28 &        5.68  &  s   &            &             \\
   5339.929 &    26 &   50 &       4.61 &         4.8 &  100 &       5.64 &        5.55 &  105 &       5.17 &        5.1  &  w   &            &              &  n   &            &             \\
   5341.024 &    26 &  115 &       4.64 &        4.35 &   s  &            &             &  145 &       4.75 &         4.9 &  130 &       4.95 &        5.22  & 130  &   4.67     &      4.92   \\
   5367.466 &    26 &   n  &            &             &   60 &       5.40 &        5.45 &   50 &       4.89 &         5.2 &  w   &            &              &  40  &   4.85     &      4.98   \\
   5383.369 &    26 &   n  &            &             &   90 &       5.57 &        5.3  &   80 &       5.07 &        5.2  &  w   &            &              &  80  &   5.20     &      5.10   \\
   5393.168 &    26 &   40 &       4.49 &         4.5 &   65 &       5.19 &        5.1  &   70 &       4.67 &        5.0  &  105 &        5.5 &        5.43  &  85  &   5.06     &      5.02   \\
   5415.199 &    26 &   45 &       4.84 &        4.9  &   45 &       5.00 &        5.1  &   70 &       5.01 &        5.32 &   85 &       5.42 &        5.68  &  55  &   4.90     &      5.00   \\
   5424.068 &    26 &   n  &            &             &   65 &       5.19 &        5.4  &  n   &            &             &  w   &            &              &  85  &   5.26     &      5.10   \\
   5497.516 &    26 &  110 &        4.5 &         4.6 &   s  &            &             &  s   &            &             &   95 &        4.5 &        4.75  & 130  &   *4.33     &      4.65   \\
   5501.465 &    26 &  115 &       4.71 &         4.7 &  105 &       5.35 &        5.25 &  s   &            &             &  135 &       5.17 &        5.38  & 150  &   5.03     &      4.85   \\
   5506.779 &    26 &  115 &        4.5 &        4.55 &   140 &       5.70 &            &  150 &       4.66 &             &  115 &       4.68 &        5.03 & 150  &    4.81    &       4.75  \\
   5569.618 &    26 &   45 &       4.57 &        4.35 &    90 &       5.53 &       5.25 &  n   &            &             &   95 &       5.34 &        5.38 &  s   &            &             \\
   5572.842 &    26 &   50 &       4.39 &        4.35 &    85 &       5.19 &            &  100 &       4.86 &        4.65 &   90 &          5 &        5.10 & 125  &    5.40    &       n     \\
   5586.756 &    26 &   70 &        4.5 &        4.25 &   s/b &            &            &  s   &            &             &  110 &       5.08 &        5.00 &  80  &    *4.50    &       4.85  \\
   5615.644 &    26 &   85 &       4.54 &         4.3 &   115 &       5.26 &       5.05 &  135 &       5.01 &         4.9 &   90 &       4.59 &        4.88 & 130  &    5.06    &       4.80  \\
   5624.542 &    26 &   25 &       4.42 &        4.35 &    45 &       5.13 &       5.15 &   n  &            &             &  w   &            &             &  85  &    5.28    &       4.90  \\
   5658.816 &    26 &   35 &        4.6 &         4.5 &    67 &       5.41 &       5.3  &   75 &       4.94 &         5.0 &   45 &       4.83 &        5.12 &  55  &    4.82    &       4.75  \\
   5956.693 &    26 &   n  &            &             &    n  &            &            &   70 &       4.96 &           5 &   n  &            &             &  s   &            &             \\
   6065.482 &    26 &   60 &       4.65 &         4.4 &    71 &       5.28 &       5.25 &  130 &       5.32 &        5.25 &   65 &       4.84 &        5.05 &  90  &    5.20    &       4.85  \\
   6136.615 &    26 &   75 &       4.51 &        4.45 &   116 &       5.59 &       5.2  &  105 &       4.59 &         4.4 &  125 &       5.28 &        4.90 & 120  &    4.96    &       4.70  \\
   6137.691 &    26 &   60 &       4.48 &        4.55 &    90 &       5.37 &       5.42 &  120 &       4.99 &        4.85 &   90 &       4.99 &        5.30 & 115  &    5.09    &       4.80  \\
   6191.558 &    26 &   60 &       4.46 &        4.45 &    95 &       5.45 &       5.30 &  105 &       4.74 &         4.8 &  110 &       5.24 &        5.00 & 120  &    5.12    &       4.85  \\
   6200.313 &    26 &   w  &            &             &   w   &            &            &   50 &       5.11 &         5.2 &  w   &            &             &   w  &            &             \\
   6213.429 &    26 &   30 &       4.59 &        4.55 &   n   &            &            &  100 &       5.25 &         5.1 &   70 &       5.33 &        5.25 &  70  &    5.07    &       4.85  \\
   6219.280 &    26 &   30 &       4.53 &        4.45 &    40 &       5.27 &       5.3  &   95 &       5.12 &           5 &  w   &            &             &  70  &    5.00    &       5.02  \\
   6230.722 &    26 &   75 &       4.52 &         4.4 &   113 &       5.54 &       5.15 &  135 &       5.03 &         4.8 &  105 &       5.01 &        4.85 & 120  &    *5.10    &       4.80  \\
   6252.555 &    26 &   75 &       4.71 &        4.55 &    85 &       5.36 &       5.15 &  125 &       5.06 &        4.85 &   90 &       5.02 &        4.90 & 110  &    5.02    &       4.75  \\
   6254.257 &    26 &   45 &       4.86 &         4.7 &   w   &            &            &   90 &       5.14 &        4.95 &   45 &       5.03 &        5.18 &  65  &    5.03    &       n     \\
   6265.134 &    26 &   40 &       4.76 &         4.7 &   n   &            &            &  100 &       5.23 &        5.00 &   55 &       5.14 &        5.00 &  70  &    5.05    &       4.95  \\
   6297.792 &    26 &   45 &       4.99 &           5 &    50 &       5.63 &        5.6 &   70 &       5.02 &        5.00 &  w   &            &             &  n   &            &            \\
   6318.018 &    26 &   40 &       4.81 &         4.8 &   n   &            &            &   90 &       5.18 &        5.00 &   45 &       5.04 &        5.25 &  75  &    5.18    &       4.95  \\
   6335.330 &    26 &   45 &       4.49 &        4.6  &    85 &       5.60 &       5.45 &  105 &       4.96 &        4.85 &   50 &       4.73 &        4.80 & 105  &    5.14    &       4.85  \\
   6344.148 &    26 &   n  &            &             &   w   &            &            &   30 &       5.02 &        5.10 &  w   &            &             &  w   &            &             \\
   6358.697 &    26 &   25 &       4.59 &         4.6 &   w   &            &            &  105 &       5.26 &        5.00 &  n   &            &             &  65  &    5.06    &       4.95  \\
   6393.600 &    26 &   75 &       4.66 &        4.45 &   105 &       5.59 &       5.30 &   s  &            &             &  135 &       5.55 &        5.28 & 115  &    5.03    &       4.80  \\
   6411.649 &    26 &   30 &       4.57 &         4.5 &    36 &       5.04 &       5.05 &   55 &       4.74 &        4.85 &   n  &            &             &  50  &    4.81    &       4.65  \\
   6421.350 &    26 &   55 &       4.56 &         4.6 &    65 &       5.26 &       5.30 &  115 &       5.02 &        4.90 &   80 &       5.03 &        4.90 &  90  &    4.89    &       4.70  \\
   6430.846 &    26 &   75 &       4.62 &         4.5 &    76 &       5.22 &       5.10 &  125 &       4.94 &        4.80 &   90 &       4.96 &        4.80 & 110  &    4.93    &       4.73  \\
   6494.980 &    26 &   80 &       4.32 &         4.3 &   126 &       5.51 &       5.10 &  140 &        4.8 &        4.75 &   90 &       4.57 &        4.45 & 115  &    4.62    &       4.55  \\
   6546.238 &    26 &   40 &       4.61 &        4.65 &    55 &       5.33 &       5.35 &   90 &          5 &        4.90 &   65 &       5.10 &        5.10 &  85  &    5.11    &       4.95  \\
   6592.913 &    26 &   55 &       4.74 &         4.6 &    80 &       5.57 &       5.40 &   85 &       4.84 &        4.80 &   50 &       4.81 &        4.85 &  90  &    5.07    &       4.80  \\
   6593.870 &    26 &   30 &       4.77 &        4.65 &   w   &            &            &   80 &       5.17 &        5.00 &   40 &       5.11 &        5.20 &  50  &    4.99    &       4.92  \\
   6677.985 &    26 &   60 &       4.62 &        4.55 &    90 &       5.52 &       5.40 &  120 &        5.1 &        4.90 &   75 &       4.94 &        4.90 &  90  &    4.88    &       4.75  \\
   4923.922 &  26.1 &   85 &       4.23 &        4.4  &   120 &       4.66 &       5.00 &  n   &            &             &  145 &       5.13 &        5.21 & 130  &    5.03    &       5.25  \\
   5018.435 &  26.1 &  100 &       4.62 &        4.55 &   s   &            &            &   n  &            &             &  130 &       4.95 &        4.95 & 145  &    5.40    &       5.22  \\
   5197.568 &  26.1 &   n  &            &             &    80 &       5.21 &       5.58 &   n  &            &             &  n   &            &             &  60  &    4.90    &       4.82  \\
   5275.997 &  26.1 &   45 &       4.43 &         4.6 &    90 &       5.16 &       4.95 &   n  &            &             &  n   &            &             &  60  &    4.69    &       4.70  \\
   5534.839 &  26.1 &   w  &            &             &   w   &            &            &   40 &       5.48 &        5.60 &  w   &            &             &  w   &            &             \\
   6456.381 &  26.1 &   n  &            &             &   35  &       5.40 &       5.45 &   35 &       5.43 &        5.45 &  w   &            &             &  35  &    5.30    &       5.15  \\
   6516.077 &  26.1 &   20 &       4.82 &       4.7   &    40 &       5.48 &       5.45 &   w  &            &             &   n  &            &             &  25  &    4.98    &       5.00  \\
   5889.951 &    11 &  \textit{215} &       \textit{3.61} &        \textit{3.39} &   
                       \textit{200} &       \textit{3.97} &        \textit{3.79} &  
                       \textit{250} &       \textit{3.64} &        \textit{3.79} &  
                       \textit{170} &       \textit{3.07} &        \textit{2.95} &  
                       \textit{195} &       \textit{3.11} &        \textit{2.79}    \\

   5895.924 &    11 &  \textit{200} &       \textit{3.71} &        \textit{3.40} &   
                       \textit{175} &       \textit{3.90} &        \textit{3.74} & 
                       \textit{200} &       \textit{3.25} &        \textit{2.99} & 
                       \textit{150} &       \textit{3.11} &        \textit{3.05} &  
                       \textit{175} &       \textit{3.14} &        \textit{2.99}    \\

   5172.684 &    12 &  \textit{255} &       \textit{5.46} &        \textit{5.25} &   
                       \textit{205} &       \textit{5.27} &        \textit{5.60} &  
                       \textit{245} &       \textit{5.12} &        n    &  
                                n   &                     &                      &   
                                n   &                     &                    \\

   5183.604 &    12 &  \textit{290} &       \textit{5.48} &         \textit{5.5} &   
                       \textit{230} &       \textit{5.34} &        \textit{5.48} &  
                       \textit{270} &       \textit{5.12} &        n    &  
                       \textit{210} &  \textit{4.75}  &  \textit{5.01} & 
                       n &
                                   &                 \\
   5528.405 &    12 &  105 &       5.82 &         5.6 &    98 &       5.73 &         5.5 &  115 &       5.65 &        5.55 &  100 &       5.62 &        5.51 & 115  &   5.80     &      5.60   \\
%   7665.    &    19 &      &        &          &      &        &          &      &        &         &      &        &         &      &            &            \\
   7698.974 &    19 &   63 &        &          &    w &        &          &  115 &        &         &   60 &        &         & 105  &   5.80     &      5.60  \\
   5265.556 &    20 &   50 &       4.34 &        4.24 &     w &            &             &    n &            &             &    n &            &             &  n   &            &             \\
   5588.749 &    20 &   65 &       4.05 &        3.84 &     n &            &             &   80 &       3.97 &        4.09 &    n &            &             &  70  &   3.99     &      3.99   \\
   5594.462 &    20 &   65 &        4.3 &        4.19 &    80 &       4.66 &        4.36 &   65 &       4.01 &        4.29 &  125 &       5.15 &       4.92  &  70  &   4.25     &      4.39   \\
   5857.451 &    20 &   45 &       4.18 &        4.12 &     w &            &             &   50 &       4.03 &        4.07 &    w &            &             &  65  &   4.39     &      4.24   \\
   6102.723 &    20 &   70 &       4.28 &        4.19 &     n &            &             &   60 &       3.83 &        3.79 &   55 &       4.12 &           4.00 &  75  &   4.22     &      4.09   \\
   6122.217 &    20 &   95 &       4.16 &        4.09 &    61 &       3.98 &        3.86 &  115 &       4.07 &        4.04 &  115 &       4.44 &         4.20 & 110  &   4.20     &      4.14   \\
   6162.173 &    20 &  130 &       4.19 &        3.84 &    86 &       3.82 &        3.64 &  105 &       3.44 &        3.29 &   95 &       3.67 &        3.55 & 120  &   3.84     &      3.59   \\
   6169.563 &    20 &   50 &       4.19 &        3.99 &     n &            &             &   60 &       4.08 &             &    n &            &             &  35  &   3.86     &      3.99   \\
   6439.075 &    20 &  100 &       4.16 &        3.89 &    40 &       3.52 &        3.44 &   90 &        3.7 &        3.69 &   85 &       3.93 &        3.65 &  90  &   3.87     &      3.74   \\
   6449.808 &    20 &   35 &       4.14 &        4.14 &     n &            &             &    n &            &             &    n &            &             &  40  &   4.19     &      4.09   \\
   6462.567 &    20 &  100 &       4.31 &        3.99 &    50 &       3.83 &        3.69 &  130 &        4.4 &        4.19 &   90 &       4.15 &         3.90 & 105  &   4.22     &      4.04   \\
   6493.781 &    20 &   65 &       3.96 &        3.89 &     w &            &             &   45 &       3.42 &        3.39 &    w &            &             &  60  &   3.79     &      3.82   \\
   6717.681 &    20 &   30 &       4.37 &        4.31 &     n &            &             &   45 &        4.4 &        4.32 &    n &            &             &  20  &   4.08     &      4.14   \\
   5526.790 &    21 &      &            &             &       &            &             &      &            &             &      &            &             &      &            &             \\        
   4981.731 &    22 &   80 &        2.2 &        2.15 &    95 &        2.9 &          n  &    n &            &             &    n &            &             & 140  &   2.86     &      2.77   \\
   4991.066 &    22 &   75 &       2.23 &        2.25 &   104 &       3.14 &         3.1 &    w &            &             &    n &            &             & 140  &   2.96     &      3.15   \\
   4999.503 &    22 &   75 &       2.34 &        2.45 &     n &            &             &  150 &       2.99 &        2.85 &    n &            &             &  95  &   2.42     &      2.43   \\
   5007.209 &    22 &   75 &       2.48 &        2.40 &   100 &       3.33 &         3.2 &    n &            &             &    n &            &             & 140  &   3.21     &      3.17   \\
   5064.653 &    22 &   55 &       2.17 &        2.47 &    78 &        3.2 &        3.15 &    n &            &             &    n &            &             &  n   &            &             \\
   5192.969 &    22 &   75 &       2.37 &        2.35 &    35 &       2.56 &             &    n &            &             &    n &            &             &  n   &            &             \\
   5210.384 &    22 &   70 &       2.21 &         2.2 &     n &            &             &  150 &       2.77 &        2.75 &    n &            &             &  n   &            &             \\
   5188.680 &  22.1 &   80 &       2.31 &         2.5 &     n &            &             &  150 &       3.62 &        3.40 &    n &            &             &  n   &            &             \\
   5226.543 &  22.1 &   95 &       2.62 &         2.3 &     n &            &             &  150 &       3.67 &         3.5 &    n &            &             &  n   &            &             \\
   5336.786 &  22.1 &   65 &        2.4 &         2.4 &     n &            &             &    n &            &             &    n &            &             &  90  &   2.79     &      2.67   \\
   6491.561 &  22.1 &   30 &       2.47 &        2.50 &     w &            &             &   40 &       2.79 &        2.77 &    n &            &             &  30  &   2.52     &      2.50   \\
   5206.023 &    24 &  115 &       2.57 &        2.45 &   155 &       3.76 &        3.65 &    n &            &             &    n &            &             &  n   &            &      n      \\
   5345.796 &    24 &   50 &       2.61 &        2.54 &    70 &       3.39 &        3.29 &  100 &       2.85 &        2.99 &  110 &       3.56 &        3.48 &  50  &   2.47     &      2.69   \\
   5409.783 &    24 &   65 &       2.57 &        2.45 &    82 &        3.3 &        3.19 &   80 &       2.33 &        2.49 &   85 &       2.95 &        3.22 &  85  &   2.67     &      2.79   \\
   5476.904 &    28 &   90 &       3.14 &        3.07 &   130 &       4.26 &        4.27 &  175 &       4.22 &        4.12 &  125 &       3.72 &        3.58 & 115  &   3.35     &      3.17   \\
   5754.656 &    28 &   w  &            &             &    40 &       4.47 &        4.67 &    w &            &             &    w &            &             &  25  &   3.57     &      3.74   \\
   6108.116 &    28 &   w  &            &             &    65 &       4.86 &        4.82 &   50 &       3.78 &        3.80 &    n &            &             &  40  &   3.82     &      3.82   \\
   6643.630 &    28 &   30 &       3.29 &        3.17 &    85 &       4.69 &        4.62 &   65 &       3.52 &        3.57 &   55 &       3.87 &        3.78 &  65  &   3.70     &      3.57   \\
   6767.772 &    28 &   w  &            &             &    72 &       4.62 &        4.67 &   70 &        3.7 &        3.65 &    w &            &             &  50  &   3.62     &      3.57   \\
   5853.690 &  56.1 &   w  &            &             &     w &            &             &   85 &      -0.34 &       -0.32 &   85 &       -0.3 &       -0.26 &  n   &            &             \\
   6141.730 &  56.1 &   55 &      -1.73 &       -1.82 &    75 &      -0.95 &       -0.92 &  115 &      -0.73 &       -0.82 &  135 &      -0.43 &       -0.44 &  70  &  -1.49     &     -1.47   \\
   6496.910 &  56.1 &   45 &      -1.76 &       -1.82 &    85 &      -0.68 &       -0.9  &  105 &       -0.8 &       -0.72 &  105 &      -0.76 &       -0.91 &  65  &  -1.44     &     -1.57   \\

\bottomrule
\end{longtable}

==> tables/5.errors.tex <==
\tabcolsep=0.16cm
\begin{table}
\caption{$\delta T$,   $\delta g$,   $\delta m$, and $\delta \xi$ are systematic errors in the stellar parameters, \teff, \logg, metallicity and microturbulence. $\sigma_{EW}$ and $\sigma_{syn}$ denotes the line scatter for the equivalent widths and syntheses methods respectively. For species with fewer than 5 lines, the scatter from \ion{Fe}{I} was adopted, and was reduced by $\sqrt{n}$ of the species. $\Delta$EW and  $\Delta$syn are the linear combinations of the line scatter and the systematic errors. }
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{species} & $\Delta T$ &   $\Delta g$ &   $\Delta m$ &   $\Delta \xi$ &  $\sigma_{EW}$ & $\sigma_{syn}$ &  $\Delta$EW &  $\Delta$syn \\
\midrule
\textbf{CB-1}    &       &       &       &       &        &           &             &       \\
\textbf{Fe I   } &  0.14 &  0.00 &  0.04 &  0.01 &   0.02 &      0.05 &        0.15 &       0.15 \\
\textbf{Fe II  } &  0.04 &  0.02 &  0.01 &  0.01 &   0.10 &      0.14 &        0.11 &       0.15 \\
\textbf{Na I   } &  0.18 &  0.01 &  0.06 &  0.03 &   0.14 &      0.17 &        0.24 &       0.26 \\
\textbf{Mg I   } &  0.10 &  0.04 &  0.03 &  0.02 &   0.11 &      0.13 &        0.16 &       0.17 \\
\textbf{\ion{K}{I}}&0.11 &  0.01 &  0.03 &  0.01 &   0.20 &      —    &        0.23 &       —    \\
\textbf{Ca I   } &  0.08 &  0.02 &  0.04 &  0.01 &   0.03 &      0.08 &        0.10 &       0.12 \\
\textbf{Sc I   } &  0.12 &  0.01 &  0.02 &  0.02 &  —     &      0.20 &          —  &       0.24 \\
\textbf{Ti I   } &  0.19 &  0.00 &  0.06 &  0.01 &   0.08 &      0.09 &        0.21 &       0.22 \\
\textbf{Ti II  } &  0.00 &  0.03 &  0.01 &  0.01 &   0.09 &      0.09 &        0.09 &       0.10 \\
\textbf{Cr I   } &  0.16 &  0.00 &  0.06 &  0.02 &   0.11 &      0.09 &        0.21 &       0.19 \\
\textbf{Ni I   } &  0.14 &  0.00 &  0.04 &  0.01 &   0.14 &      0.12 &        0.20 &       0.19 \\
\textbf{Ba II  } &  0.05 &  0.04 &  0.02 &  0.01 &   0.14 &      0.13 &        0.15 &       0.14 \\
\midrule
\textbf{CB-2}    &       &       &       &       &        &           &             &       \\
\textbf{Fe I   } &  0.10 &  0.01 &  0.03 &  0.02 &   0.03 &      0.05 &        0.12 &       0.12 \\
\textbf{Fe II  } &  0.00 &  0.05 &  0.02 &  0.01 &   0.10 &      0.14 &        0.11 &       0.15 \\
\textbf{Na I   } &  0.11 &  0.02 &  0.08 &  0.05 &   0.16 &      0.29 &        0.22 &       0.33 \\
\textbf{Mg I   } &  0.09 &  0.03 &  0.04 &  0.04 &   0.13 &      0.25 &        0.17 &       0.28 \\
\textbf{\ion{K}{I}}& —   &  —    &  —    &  —    &   —    &      —    &        —    &       —    \\
\textbf{Ca I   } &  0.07 &  0.01 &  0.01 &  0.01 &   0.10 &      0.13 &        0.12 &       0.15 \\
\textbf{Sc I   } &  0.09 &  0.01 &  0.02 &  0.01 &      — &      0.20 &           — &       0.22 \\
\textbf{Ti I   } &  0.12 &  0.01 &  0.04 &  0.02 &   0.10 &      0.15 &        0.16 &       0.20 \\
\textbf{Ti II  } &  0.03 &  0.05 &  0.02 &  0.02 &   0.23 &      0.41 &        0.23 &       0.41 \\
\textbf{Cr I   } &  0.12 &  0.02 &  0.04 &  0.03 &   0.13 &      0.27 &        0.18 &       0.30 \\
\textbf{Ni I   } &  0.12 &  0.01 &  0.03 &  0.02 &   0.10 &      0.11 &        0.16 &       0.17 \\
\textbf{Ba II  } &  0.07 &  0.06 &  0.03 &  0.00 &   0.16 &      0.17 &        0.18 &       0.19 \\
\midrule
\textbf{UMaI-1}    &       &       &       &       &        &           &             &       \\
\textbf{Fe I   } &  0.11 &  0.01 &  0.02 &  0.02 &   0.03 &      0.07 &        0.12 &       0.13 \\
\textbf{Fe II  } &  0.05 &  0.04 &  0.02 &  0.01 &   0.13 &      0.16 &        0.15 &       0.17 \\
\textbf{Na I   } &  0.14 &  0.01 &  0.03 &  0.04 &   0.13 &      0.61 &        0.20 &       0.63 \\
\textbf{Mg I   } &  0.09 &  0.02 &  0.02 &  0.02 &   0.11 &      0.34 &        0.14 &       0.35 \\
\textbf{\ion{K}{I}}&0.12 &  0.02 &  0.03 &  0.01 &   0.18 &      —    &        0.22 &           — \\
\textbf{Ca I   } &  0.09 &  0.00 &  0.02 &  0.01 &   0.10 &      0.27 &        0.14 &       0.29 \\
\textbf{Sc I   } &  0.12 &  0.00 &  0.03 &  0.01 &      — &      0.20 &          —  &       0.24 \\
\textbf{Ti I   } &  0.19 &  0.03 &  0.04 &  0.04 &   0.13 &      1.01 &        0.24 &       1.03 \\
\textbf{Ti II  } &  0.01 &  0.04 &  0.01 &  0.03 &   0.11 &      0.33 &        0.12 &       0.33 \\
\textbf{Cr I   } &  0.15 &  0.01 &  0.04 &  0.01 &   0.13 &       0.4 &        0.21 &       0.43 \\
\textbf{Ni I   } &  0.10 &  0.01 &  0.01 &  0.02 &   0.09 &      0.34 &        0.14 &       0.36 \\
\textbf{Ba II  } &  0.02 &  0.05 &  0.02 &  0.02 &   0.11 &      0.31 &        0.12 &       0.32 \\
\midrule
\textbf{UMaI-2}    &       &       &       &       &        &           &             &       \\
\textbf{Fe I   } &  0.19 &  0.03 &  0.01 &  0.02 &   0.04 &      0.06 &        0.20 &       0.20 \\
\textbf{Fe II  } &  0.03 &  0.01 &  0.00 &  0.03 &   0.16 &      0.23 &        0.17 &       0.23 \\
\textbf{Na I   } &  0.21 &  0.04 &  0.01 &  0.02 &   0.20 &      0.38 &        0.29 &       0.44 \\
\textbf{Mg I   } &  0.16 &  0.02 &  0.01 &  0.01 &   0.16 &      0.36 &        0.23 &       0.40 \\
\textbf{\ion{K}{I}}&0.12 &  0.02 &  0.01 &  0.01 &   0.28 &      —    &        0.30 &       —    \\
\textbf{Ca I   } &  0.12 &  0.02 &  0.01 &  0.01 &   0.11 &      0.17 &        0.16 &       0.21 \\
\textbf{Sc I   } &  0.14 &  0.02 &  0.01 &  0.02 &      — &      0.20 &           — &       0.24 \\
\textbf{\ion{Ti}{I}}& —   &  —    &  —    &  —    &   —    &      —    &        —    &       —    \\
\textbf{\ion{Ti}{II}}& —   &  —    &  —    &  —    &   —    &      —    &        —    &       —    \\
\textbf{Cr I   } &  0.19 &  0.03 &  0.01 &  0.02 &   0.20 &      0.29 &        0.27 &       0.35 \\
\textbf{Ni I   } &  0.18 &  0.03 &  0.01 &  0.02 &   0.20 &      0.19 &        0.27 &       0.27 \\
\textbf{Ba II  } &  0.03 &  0.02 &  0.01 &  0.04 &   0.16 &      0.16 &        0.17 &       0.17 \\
\midrule
\textbf{BooI-2}    &       &       &       &       &        &           &             &       \\
\textbf{Fe I   } &  0.12 &  0.00 &  0.06 &  0.02 &   0.03 &      0.06 &        0.14 &       0.15 \\
\textbf{Fe II  } &  0.04 &  0.02 &  0.01 &  0.02 &   0.08 &       0.1 &        0.10 &       0.11 \\
\textbf{Na I   } &  0.15 &  0.01 &  0.07 &  0.03 &   0.15 &      0.21 &        0.22 &       0.27 \\
\textbf{Mg I   } &  0.07 &  0.01 &  0.06 &  0.02 &   0.21 &      0.22 &        0.23 &       0.24 \\
\textbf{\ion{K}{I}}&0.11 &  0.00 &  0.05 &  0.01 &   0.21 &      —    &        0.24 &       —    \\
\textbf{Ca I   } &  0.08 &  0.01 &  0.04 &  0.01 &   0.06 &      0.12 &        0.11 &       0.15 \\
\textbf{Sc I   } &  0.12 &  0.00 &  0.02 &  0.02 &      — &      0.20 &           — &       0.24 \\
\textbf{Ti I   } &  0.17 &  0.00 &  0.08 &  0.03 &   0.10 &       0.2 &        0.21 &       0.27 \\
\textbf{Ti II  } &  0.01 &  0.02 &  0.03 &  0.01 &   0.15 &      0.36 &        0.15 &       0.36 \\
\textbf{Cr I   } &  0.14 &  0.00 &  0.06 &  0.01 &   0.15 &      0.17 &        0.21 &       0.23 \\
\textbf{Ni I   } &  0.12 &  0.00 &  0.04 &  0.01 &   0.09 &      0.13 &        0.16 &       0.18 \\
\textbf{Ba II  } &  0.03 &  0.03 &  0.04 &  0.01 &   0.15 &      0.16 &        0.16 &       0.17 \\
\bottomrule
\end{tabular}
\label{tab:errorsfull}
\end{table}



% \begin{table}
% \ContinuedFloat
% \caption{}
% \begin{tabular}{lrrrrrrrr}
% \toprule
% \textbf{species} & $\Delta T$ &   $\Delta g$ &   $\Delta m$ &   $\Delta \xi$ &  $\sigma_{EW}$ & $\sigma_{syn}$ &  $\Delta$EW &  $\Delta$syn \\
% \midrule
% \textbf{BooI-2}    &       &       &       &       &        &           &             &       \\
% \textbf{Fe I   } &  0.12 &  0.00 &  0.06 &  0.02 &   0.03 &      0.06 &        0.14 &       0.15 \\
% \textbf{Fe II  } &  0.04 &  0.02 &  0.01 &  0.02 &   0.08 &       0.1 &        0.10 &       0.11 \\
% \textbf{Na I   } &  0.15 &  0.01 &  0.07 &  0.03 &   0.15 &      0.21 &        0.22 &       0.27 \\
% \textbf{Mg I   } &  0.07 &  0.01 &  0.06 &  0.02 &   0.21 &      0.22 &        0.23 &       0.24 \\
% \textbf{\ion{K}{I}}&0.11 &  0.00 &  0.05 &  0.01 &   0.21 &      —    &        0.24 &       —    \\
% \textbf{Ca I   } &  0.08 &  0.01 &  0.04 &  0.01 &   0.06 &      0.12 &        0.11 &       0.15 \\
% \textbf{Sc I   } &  0.12 &  0.00 &  0.02 &  0.02 &      — &      0.20 &           — &       0.24 \\
% \textbf{Ti I   } &  0.17 &  0.00 &  0.08 &  0.03 &   0.10 &       0.2 &        0.21 &       0.27 \\
% \textbf{Ti II  } &  0.01 &  0.02 &  0.03 &  0.01 &   0.15 &      0.36 &        0.15 &       0.36 \\
% \textbf{Cr I   } &  0.14 &  0.00 &  0.06 &  0.01 &   0.15 &      0.17 &        0.21 &       0.23 \\
% \textbf{Ni I   } &  0.12 &  0.00 &  0.04 &  0.01 &   0.09 &      0.13 &        0.16 &       0.18 \\
% \textbf{Ba II  } &  0.03 &  0.03 &  0.04 &  0.01 &   0.15 &      0.16 &        0.16 &       0.17 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/6.linelist_NLTE_corr.tex <==

\begin{longtable}{rrrrrrrrrrrrr}

\caption{NLTE corrections from two databases, Inspect and MPIA, as well as \ion{Ba}{II} corrections from \citet{Mashonkina2019} and \ion{K}{I} corrections from \citet{Andrievsky10}, both marked with a '*' in the INSPECT column. }
           &        &  &    \multicolumn{2}{c}{CB-1 }   &       \multicolumn{2}{c}{CB-2 }    & \multicolumn{2}{c}{UMaI-1 }        & \multicolumn{2}{c}{UMaI-2 }    & \multicolumn{2}{c}{BooI-2 }    \\
 \cmidrule(lr){3-4}\cmidrule(lr){5-6} \cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
 wavelength &    ID &  Inspect  &  MPIA  &         Inspect  &  MPIA  &          Inspect &  MPIA  &         Inspect  &  MPIA  &         Inspect  &  MPIA   \\
\midrule
   4871.318 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4872.138 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4890.755 &  26.0 &           &  0.231 &                  &        &                  &        &                  &        &                  &  0.133        \\
   4891.492 &  26.0 &           &  0.217 &                  &        &                  &        &                  &        &                  &  0.138        \\
   4918.994 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4920.502 &  26.0 &     0.124 &        &            0.074 &        &                  &        &                  &        &          0.065   &               \\
   4939.687 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4966.089 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4994.130 &  26.0 &     0.141 &  0.201 &            0.224 &  0.153 &                  &        &                  &        &          0.195   &  0.138        \\
   5006.119 &  26.0 &           &  0.211 &                  &        &                  &        &                  &        &                  &  0.169        \\
   5012.068 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5041.072 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5041.756 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5049.819 &  26.0 &           &  0.224 &                  &        &                  &        &                  &        &                  &  0.156        \\
   5051.635 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5068.766 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5110.413 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5123.720 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5127.360 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5150.840 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5151.911 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5191.454 &  26.0 &           &  0.222 &                  &  0.143 &                  &        &                  &        &                  &               \\
   5192.344 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5194.942 &  26.0 &           &  0.206 &                  &        &                  &        &                  &        &                  &               \\
   5198.711 &  26.0 &     0.084 &  0.192 &                  &        &                  &        &                  &        &                  &               \\
   5202.336 &  26.0 &           &        &                  &        &                  &        &                  &  0.167 &                  &               \\
   5216.274 &  26.0 &     0.147 &  0.205 &                  &        &                  &        &            0.185 &  0.155 &                  &               \\
   5232.940 &  26.0 &     0.074 &  0.236 &            0.062 &  0.057 &                  &        &            0.099 &  0.107 &          0.064   &  0.127        \\
   5247.050 &  26.0 &     0.130 &  0.198 &                  &        &            0.159 &  0.138 &            0.174 &  0.170 &          0.159   &  0.147        \\
   5250.210 &  26.0 &     0.145 &  0.094 &                  &        &            0.152 &  0.064 &            0.173 &  0.084 &                  &  0.069        \\
   5250.646 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5254.956 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5266.555 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5281.790 &  26.0 &     0.096 &  0.201 &            0.149 &  0.170 &                  &        &            0.117 &  0.180 &          0.071   &  0.173        \\
   5283.621 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5307.361 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5324.179 &  26.0 &           &  0.234 &                  &        &                  &        &                  &  0.159 &                  &  0.157        \\
   5328.532 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5332.900 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &              \\
   5339.929 &  26.0 &           &  0.192 &                  &  0.164 &                  &  0.127 &                  &        &                  &  0.155        \\
   5341.024 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5367.466 &  26.0 &           &        &                  &  0.206 &                  &  0.184 &                  &        &                  &  0.172        \\
   5383.369 &  26.0 &           &        &            0.188 &  0.230 &            0.127 &  0.211 &                  &        &          0.113   &  0.212        \\
   5393.168 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5415.199 &  26.0 &           &  0.224 &                  &  0.230 &                  &  0.210 &                  &  0.231 &                  &  0.204        \\
   5424.068 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5497.516 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5501.465 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5506.779 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5569.618 &  26.0 &           &  0.195 &                  &  0.164 &                  &        &                  &  0.173 &                  &               \\
   5572.842 &  26.0 &           &  0.202 &                  &  0.159 &                  &  0.112 &                  &  0.174 &                  &  0.164        \\
   5586.756 &  26.0 &     0.125 &  0.220 &                  &        &                  &        &            0.106 &  0.170 &          0.078   &  0.167        \\
   5615.644 &  26.0 &           &  0.220 &                  &  0.146 &                  &  0.101 &                  &  0.167 &                  &  0.157       \\
   5624.542 &  26.0 &           &  0.191 &                  &  0.169 &                  &        &                  &        &                  &  0.146        \\
   5658.816 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5956.693 &  26.0 &           &        &                  &        &            0.100 &  0.126 &            0.130 &  0.167 &                  &               \\
   6065.482 &  26.0 &     0.087 &  0.200 &            0.145 &  0.159 &            0.081 &  0.111 &            0.128 &  0.164 &          0.093   &  0.147        \\
   6136.615 &  26.0 &           &  0.170 &                  &  0.114 &                  &  0.045 &                  &  0.117 &                  &  0.093        \\
   6137.691 &  26.0 &           &  0.164 &                  &  0.113 &                  &  0.045 &                  &  0.117 &                  &  0.092        \\
   6191.558 &  26.0 &           &  0.210 &                  &  0.157 &                  &  0.098 &                  &  0.166 &                  &  0.154        \\
   6200.313 &  26.0 &           &        &                  &        &            0.070 &  0.119 &                  &        &                  &               \\
   6213.429 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6219.280 &  26.0 &     0.099 &        &            0.156 &        &            0.088 &        &                  &        &          0.088   &               \\
   6230.722 &  26.0 &           &  0.213 &                  &  0.150 &                  &  0.084 &                  &  0.163 &                  &  0.152        \\
   6252.555 &  26.0 &     0.106 &  0.204 &            0.176 &  0.163 &            0.108 &  0.116 &            0.145 &  0.167 &          0.104   &  0.152        \\
   6254.257 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6265.134 &  26.0 &     0.092 &  0.198 &                  &        &            0.088 &  0.126 &            0.124 &  0.165 &          0.085   &  0.141        \\
   6297.792 &  26.0 &     0.091 &  0.195 &            0.123 &  0.165 &            0.084 &  0.123 &                  &        &                  &               \\
   6318.018 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6335.330 &  26.0 &           &  0.201 &                  &  0.165 &                  &  0.126 &                  &  0.167 &                  &  0.146        \\
   6344.148 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6358.697 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6393.600 &  26.0 &           &  0.222 &                  &  0.166 &                  &        &                  &  0.175 &                  &  0.163        \\
   6411.649 &  26.0 &           &  0.203 &                  &  0.174 &                  &  0.140 &                  &        &                  &  0.155        \\
   6421.350 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6430.846 &  26.0 &     0.108 &        &            0.158 &        &            0.114 &        &            0.147 &        &          0.113   &               \\
   6494.980 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6546.238 &  26.0 &           &  0.202 &                  &  0.161 &                  &  0.120 &                  &  0.166 &                  &  0.146        \\
   6592.913 &  26.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6593.870 &  26.0 &     0.085 &        &                  &        &            0.068 &        &            0.112 &        &          0.078   &               \\
   6677.985 &  26.0 &           &  0.206 &                  &  0.157 &                  &  0.106 &                  &  0.165 &                  &  0.150        \\
   4923.922 &  26.1 &    -0.150 &  0.089 &           -0.040 &  0.071 &                  &        &           -0.042 &  0.076 &          -0.04   &  0.092        \\
   5018.435 &  26.1 &    -0.020 &        &                  &        &                  &        &           -0.036 &        &          -0.066  &               \\
   5197.568 &  26.1 &           &        &           -0.009 &  0.001 &                  &        &                  &        &          -0.009  &  0.002        \\
   5275.997 &  26.1 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5534.839 &  26.1 &           &        &                  &        &                  &  0.002 &                  &        &                  &               \\
   6456.381 &  26.1 &           &        &           -0.004 &        &           -0.007 &        &                  &        &          -0.008  &               \\
   6516.077 &  26.1 &    -0.005 &        &           -0.003 &        &                  &        &           -0.006 &        &          -0.006  &               \\
   5889.951 &  11.0 &    -0.264 &        &           -0.496 &        &           -0.094 &        &           -0.268 &        &          -0.208  &               \\
   5895.924 &  11.0 &    -0.289 &        &           -0.452 &        &           -0.127 &        &           -0.205 &        &          -0.197  &               \\
   5172.684 &  12.0 &    -0.001 &  0.068 &           -0.049 &  0.070 &                  &  0.066 &                  &  0.059 &                  &               \\
   5183.604 &  12.0 &     0.006 &  0.066 &           -0.028 &  0.077 &                  &  0.070 &                  &  0.066 &                  &               \\
   5528.405 &  12.0 &    -0.071 &  0.099 &            0.002 &  0.022 &                  & -0.001 &                  &  0.050 &          -0.08   &  0.057        \\
%   7665.    &    19 &           &        &                  &        &                  &        &                  &        &                  &               \\
   7698.974 &    19 &    *0.210 &        &           *0.330 &        &           *0.210 &        &           *0.210 &        &          *0.210  &               \\
   5265.556 &  20.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5588.749 &  20.0 &           &  0.269 &                  &        &                  &  0.218 &                  &  0.273 &                  &  0.231        \\
   5594.462 &  20.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5857.451 &  20.0 &           &  0.147 &                  &        &                  &  0.114 &                  &  0.150 &                  &  0.120        \\
   6102.723 &  20.0 &           &  0.218 &                  &        &                  &  0.206 &                  &  0.243 &                  &  0.204        \\
   6122.217 &  20.0 &           &  0.209 &                  &  0.180 &                  &  0.143 &                  &  0.211 &                  &  0.197        \\
   6162.173 &  20.0 &           &  0.212 &                  &  0.129 &                  &  0.091 &                  &  0.188 &                  &  0.181        \\
   6169.563 &  20.0 &           &  0.086 &                  &        &                  &  0.086 &                  &        &                  &  0.077        \\
   6439.075 &  20.0 &           &  0.169 &                  &  0.129 &                  &  0.060 &                  &  0.165 &                  &  0.134        \\
   6449.808 &  20.0 &           &  0.000 &                  &        &                  &  0.000 &                  &        &                  &               \\
   6462.567 &  20.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6493.781 &  20.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6717.681 &  20.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5526.790 &  21.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   4981.731 &  22.0 &     0.294 &  0.408 &            0.125 &  0.341 &                  &        &                  &        &          0.209   &  0.368        \\
   4991.066 &  22.0 &     0.345 &  0.427 &            0.148 &  0.367 &                  &        &                  &        &          0.220   &  0.384        \\
   4999.503 &  22.0 &     0.375 &  0.514 &                  &        &            0.203 &  0.370 &                  &        &          0.304   &  0.449        \\
   5007.209 &  22.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5064.653 &  22.0 &           &  0.484 &                  &  0.569 &                  &        &                  &        &                  &               \\
   5192.969 &  22.0 &           &  0.490 &                  &  0.583 &                  &        &                  &        &                  &               \\
   5210.384 &  22.0 &           &  0.480 &                  &        &                  &  0.574 &                  &        &                  &               \\
   5188.680 &  22.1 &           &  0.096 &                  & -0.079 &                  & -0.108 &                  &        &                  &               \\
   5226.543 &  22.1 &           &  0.097 &                  &        &                  & -0.081 &                  &        &                  &               \\
   5336.786 &  22.1 &           &  0.103 &                  &        &                  &        &                  &        &                  &  0.089        \\
   6491.561 &  22.1 &           &  0.042 &                  &        &                  &  0.038 &                  &        &                  &  0.056        \\
   5206.023 &  24.0 &           &  0.530 &                  &  0.306 &                  &        &                  &        &                  &               \\
   5345.796 &  24.0 &           &  0.415 &                  &  0.413 &                  &  0.355 &                  &  0.410 &                  &  0.388        \\
   5409.783 &  24.0 &           &  0.417 &                  &  0.397 &                  &  0.307 &                  &  0.406 &                  &  0.397        \\
   4823.514 &  25.0 &           &        &                  &  0.525 &                  &        &                  &  0.537 &                  &               \\
   5476.904 &  28.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5754.656 &  28.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6108.116 &  28.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6643.630 &  28.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   6767.772 &  28.0 &           &        &                  &        &                  &        &                  &        &                  &               \\
   5853.690 &  56.1 &           &        &                  &        &            *0.10 &        &                  &        &            *0.10 &               \\
   6141.730 &  56.1 &     *0.12 &        &            *0.07 &        &            *0.13 &        &            *0.07 &        &            *0.13 &               \\
   6496.910 &  56.1 &     *0.05 &        &            *0.01 &        &            *0.05 &        &            *0.03 &        &            *0.05 &               \\
\bottomrule
\label{tab:nltefull}
\end{longtable}

==> tables/7.abundances.tex <==

\begin{table*}
\caption{Scaled-solar chemical abundances from our EW analyses, except for species labelled with an * which are from syntheses, with and without NLTE corrections (in Table~\ref{tab:nltestub}). Metallicity [Fe/H] is a weighted mean of [\ion{Fe}{I}/H] and [\ion{Fe}{II}/H]. Solar abundances as 12+log(X/H) from \citet{Asplund09}, and [X/Fe] = log(X/Fe)$_*$ $-$ log(X/Fe)$_\odot$. Species such as \ion{Ni}{I} which have no available NLTE corrections still show an altered value in the NLTE table, which is strictly due to the \ion{Fe}{} NLTE corrections.}
\begin{tabular}{lrrrrrr}
\toprule
                          & Solar&                   CB-1 &                     CB-2 &                  UMaI-1 &                 UMaI-2 &                   BooI-2 \\
                     &  log(X/H) &                [X/Fe]  &            [X/Fe]        &         [X/Fe]          &                [X/Fe]  &           [X/Fe]         \\
\midrule
\textbf{LTE} \\
% \\
\textrm{[Fe/H]}           & 7.50 &  -2.88$\pm$0.15    (77) &  -2.17$\pm$0.12    (46) &  -2.49$\pm$0.12    (44) &  -2.42$\pm$0.20    (45) &  -2.49$\pm$0.14    (61) \\
\textrm{[\ion{Fe}{I}/H]}  & 7.50 &  -2.88$\pm$0.15    (73) &  -2.15$\pm$0.12    (41) &  -2.51$\pm$0.12    (42) &  -2.42$\pm$0.20    (43) &  -2.49$\pm$0.14    (55) \\
\textrm{[\ion{Fe}{II}/H]} & 7.50 &  -2.97$\pm$0.11 \ \ (4) &  -2.32$\pm$0.11 \ \ (5) &  -2.04$\pm$0.15 \ \ (2) &  -2.46$\pm$0.17 \ \ (2) &  -2.45$\pm$0.10 \ \ (6) \\
\textrm{[\ion{Na}{I}/Fe]} & 6.24 &   0.30$\pm$0.24 \ \ (2) &  -0.13$\pm$0.22 \ \ (2) &  -0.30$\pm$0.20 \ \ (2) &  -0.73$\pm$0.29 \ \ (2) &  -0.63$\pm$0.22 \ \ (2) \\
\textrm{[\ion{Mg}{I}/Fe]} & 7.60 &   0.87$\pm$0.16 \ \ (3) &   0.02$\pm$0.17 \ \ (3) &   0.19$\pm$0.14 \ \ (3) &   0.44$\pm$0.23 \ \ (1) &   0.69$\pm$0.23 \ \ (1) \\
\textrm{[\ion{K}{I}/Fe]}  & 5.03 &   0.65$\pm$0.23 \ \ (1) &  <0.28$\pm$0.23 \ \ (1) &   0.55$\pm$0.24 \ \ (1) &   0.26$\pm$0.23 \ \ (1) &   0.64$\pm$0.24 \ \ (1) \\
\textrm{[\ion{Ca}{I}/Fe]} & 6.34 &   0.74$\pm$0.10    (13) &  -0.21$\pm$0.12 \ \ (5) &   0.09$\pm$0.14    (11) &   0.32$\pm$0.16 \ \ (6) &   0.22$\pm$0.11    (12) \\
\textrm{[\ion{Sc}{I}/Fe]*}& 3.13 &  -0.10$\pm$0.24 \ \ (1) &   0.00$\pm$0.22 \ \ (1) &   0.70$\pm$0.24 \ \ (1) &   0.00$\pm$0.24 \ \ (1) &   0.10$\pm$0.24 \ \ (1) \\
\textrm{[\ion{Ti}{I}/Fe]} & 4.95 &   0.22$\pm$0.21 \ \ (7) &   0.25$\pm$0.16 \ \ (5) &   0.42$\pm$0.24 \ \ (2) &           —    \ \     (0) &   0.40$\pm$0.21 \ \ (4) \\
\textrm{[\ion{Ti}{II}/Fe]}& 4.95 &   0.38$\pm$0.09 \ \ (4) &               — \ \ (0) &   0.90$\pm$0.12 \ \ (3) &           —    \ \     (0) &   0.20$\pm$0.15 \ \ (2) \\
\textrm{[\ion{Cr}{I}/Fe]} & 5.64 &  -0.18$\pm$0.21 \ \ (3) &   0.01$\pm$0.18 \ \ (3) &  -0.56$\pm$0.21 \ \ (2) &   0.03$\pm$0.27 \ \ (2) &  -0.58$\pm$0.21 \ \ (2) \\
\textrm{[\ion{Ni}{I}/Fe]} & 6.22 &  -0.13$\pm$0.20 \ \ (2) &   0.53$\pm$0.16 \ \ (5) &   0.07$\pm$0.14 \ \ (4) &  -0.01$\pm$0.27 \ \ (2) &  -0.12$\pm$0.16 \ \ (5) \\
\textrm{[\ion{Ba}{II}/Fe]}& 2.18 &  -1.10$\pm$0.15 \ \ (2) &  -0.95$\pm$0.18 \ \ (2) &  -0.39$\pm$0.12 \ \ (3) &  -0.43$\pm$0.17 \ \ (3) &  -1.20$\pm$0.16 \ \ (2) \\
\\
\textbf{NLTE }               \\
\textrm{[Fe/H]}           & 7.50 &  -2.69$\pm$0.15    (77) &  -2.02$\pm$0.12    (46) &  -2.37$\pm$0.12    (44) &  -2.27$\pm$0.20    (45) &  -2.35$\pm$0.14    (61) \\
\textrm{[\ion{Fe}{I}/H]}  & 7.50 &  -2.68$\pm$0.15    (73) &  -1.99$\pm$0.12    (41) &  -2.39$\pm$0.12    (42) &  -2.26$\pm$0.20    (43) &  -2.34$\pm$0.14    (55) \\
\textrm{[\ion{Fe}{II}/H]} & 7.50 &  -2.88$\pm$0.11 \ \ (4) &  -2.28$\pm$0.11 \ \ (5) &  -2.04$\pm$0.15 \ \ (2) &  -2.38$\pm$0.17 \ \ (2) &  -2.40$\pm$0.10 \ \ (6) \\
\textrm{[\ion{Na}{I}/Fe]} & 6.24 &  -0.17$\pm$0.24 \ \ (2) &  -0.75$\pm$0.22 \ \ (2) &  -0.53$\pm$0.20 \ \ (2) &  -1.12$\pm$0.29 \ \ (2) &  -0.97$\pm$0.22 \ \ (2) \\
\textrm{[\ion{Mg}{I}/Fe]} & 7.60 &   0.76$\pm$0.16 \ \ (3) &  -0.07$\pm$0.17 \ \ (3) &   0.12$\pm$0.14 \ \ (3) &   0.35$\pm$0.23 \ \ (1) &   0.61$\pm$0.23 \ \ (1) \\
\textrm{[\ion{K}{I}/Fe]}  & 5.03 &   0.19$\pm$0.23 \ \ (1) & <-0.20$\pm$0.23 \ \ (1) &   0.23$\pm$0.24 \ \ (1) &   -0.1$\pm$0.23 \ \ (1) &   0.29$\pm$0.24 \ \ (1) \\
\textrm{[\ion{Ca}{I}/Fe]} & 6.34 &   0.74$\pm$0.10    (13) &  -0.21$\pm$0.12 \ \ (5) &   0.10$\pm$0.14    (11) &   0.37$\pm$0.16 \ \ (6) &   0.24$\pm$0.11    (12) \\
\textrm{[\ion{Sc}{I}/Fe]*}& 3.13 &  -0.30$\pm$0.20 \ \ (1) &  -0.20$\pm$0.20 \ \ (1) &   0.50$\pm$0.20 \ \ (1) &  -0.20$\pm$0.20 \ \ (1) &  -0.10$\pm$0.20 \ \ (1) \\
\textrm{[\ion{Ti}{I}/Fe]} & 4.95 &   0.50$\pm$0.21 \ \ (7) &   0.57$\pm$0.17 \ \ (5) &   0.77$\pm$0.25 \ \ (2) &          —                \ \ (0) &   0.66$\pm$0.21 \ \ (4) \\
\textrm{[\ion{Ti}{II}/Fe]}& 4.95 &   0.27$\pm$0.09 \ \ (4) &               — \ \ (0) &   0.73$\pm$0.12 \ \ (3) &         —      \ \ (0) &   0.13$\pm$0.15 \ \ (2) \\
\textrm{[\ion{Cr}{I}/Fe]} & 5.64 &   0.08$\pm$0.21 \ \ (3) &   0.23$\pm$0.18 \ \ (3) &  -0.35$\pm$0.21 \ \ (2) &   0.29$\pm$0.27 \ \ (2) &  -0.33$\pm$0.21 \ \ (2) \\
\textrm{[\ion{Ni}{I}/Fe]} & 6.22 &  -0.32$\pm$0.20 \ \ (2) &   0.38$\pm$0.16 \ \ (5) &  -0.05$\pm$0.14 \ \ (4) &  -0.16$\pm$0.27 \ \ (2) &  -0.26$\pm$0.16 \ \ (5) \\
\textrm{[\ion{Ba}{II}/Fe]}& 2.18 &  -1.20$\pm$0.15 \ \ (2) &  -1.06$\pm$0.18 \ \ (2) &  -0.41$\pm$0.12 \ \ (3) &  -0.53$\pm$0.17 \ \ (3) &  -1.25$\pm$0.16 \ \ (2) \\
\bottomrule
\end{tabular}
\label{tab:figureabuns}
\end{table*}

==> tables/8.full_member_list.tex <==
\begin{landscape}

%[KCG2013] UmaI 97 707

\begin{longtable}{lrllrrrrrrrllllllll}
\caption{Stellar sample selected from \citet{McVenn2020} are identified by their Gaia IDs.  Stars with spectroscopic analyses are identified with given Starnames, including their published radial velocities RVs and metallicities [Fe/H].  See references below.  We have calculated their radius, R/R$_h$, using parameters in Table~\ref{tab:galpar}. Sources for Fe and RV: 
m: \citet{Kleyna05},
o: \citet{Martin07}, 
b: \citet{Feltzing09}, 
c: \citet{Frebel10}, 
d: \citet{Norris10a}, 
e: \citet{Lai11}, 
f: \citet{Gilmore13}, 
g: \citet{Vargas13}, 
h: \citet{Ishigaki14},  
i: \citet{Frebel16}, 
n: \citet{Longeard22}
p: \citet{Jenkins21}.
% We do not replace data with L21, but we will fill in missing data with L21 if any.
Just RV: j:\citet{Simon2007}, 
k: \citet{Koposov11}, 
l: \citet{Munoz06}.}. 
\label{tab:allgalstars}
\\
\toprule
{} &            source\_id &      UFD &                  Starname &  RA (J2016) &  Dec (J2016) &   R/R$_h$ &      RV &      G &  BP-RP &  PSAT &  [Fe/H] &   source \\
\midrule
\textbf{0  } &  3959869107138861056 &  Com Ber &                 ComBer-S1 &   186.68111 &     23.95070 &  0.81 &   93.80 &  17.89 &   1.07 &  1.00 &   -2.31 &      c,g \\
\textbf{1  } &  3959874634761012224 &  Com Ber &                 ComBer-S2 &   186.73107 &     23.93605 &  0.45 &   96.40 &  17.79 &   1.05 &  1.00 &   -2.88 &      c,g \\
\textbf{2  } &  3959873883142494720 &  Com Ber &                 ComBer-S3 &   186.73609 &     23.93661 &  0.47 &   99.00 &  17.25 &   1.12 &  1.00 &   -2.53 &      c,g \\
\textbf{3  } &  3959867144338018304 &  Com Ber &                         — &   186.68810 &     23.84574 &  1.32 &  106.11 &  19.89 &   1.04 &  0.75 &   -2.92 &        g \\
\textbf{4  } &  3959867728453587968 &  Com Ber &                         — &   186.73948 &     23.89943 &  0.12 &   96.27 &  19.15 &   0.99 &  1.00 &   -3.38 &        g \\
\textbf{5  } &  3959867865892540928 &  Com Ber &                         — &   186.69726 &     23.89887 &  0.60 &   91.07 &  20.22 &   0.79 &  0.97 &   -3.01 &        g \\
\textbf{6  } &  3959869755678143488 &  Com Ber &                         — &   186.88803 &     23.87207 &  1.53 &   89.05 &  19.53 &   0.84 &  0.93 &   -2.65 &        g \\
\textbf{7  } &  3959888309936927744 &  Com Ber &                         — &   186.62087 &     24.06772 &  2.36 &   98.47 &  20.31 &   0.94 &  0.87 &   -2.52 &        g \\
\textbf{8  } &  3959870477232655360 &  Com Ber &                         — &   186.83611 &     23.89460 &  1.00 &   89.14 &  20.49 &   1.03 &  0.34 &   -2.87 &        g \\
\textbf{9  } &  3959868763541740544 &  Com Ber &                         — &   186.71194 &     23.93341 &  0.47 &   93.27 &  18.61 &   0.33 &  1.00 &       — &        j \\
\textbf{10 } &  3959869240282051584 &  Com Ber &                         — &   186.85563 &     23.82725 &  1.36 &  113.69 &  19.01 &   0.05 &  1.00 &       — &        j \\
\textbf{11 } &  3959870722046625280 &  Com Ber &                         — &   186.80574 &     23.91066 &  0.74 &   91.59 &  20.63 &   0.36 &  0.53 &       — &        j \\
\textbf{12 } &  3959874909638929920 &  Com Ber &                         — &   186.70903 &     23.96174 &  0.82 &  101.27 &  20.34 &   0.89 &  0.96 &       — &        j \\
\textbf{13 } &  3959887828900577280 &  Com Ber &                         — &   186.63371 &     24.02378 &  1.79 &   99.99 &  18.56 &   0.17 &  1.00 &       — &        j \\
\textbf{14 } &  3959847524927441920 &  Com Ber &                         — &   187.10271 &     23.94040 &  4.41 &       — &  18.73 &   0.95 &  0.96 &       — &        — \\
\textbf{15 } &  3959847593646920704 &  Com Ber &                         — &   187.13073 &     23.94670 &  4.78 &       — &  18.66 &   1.02 &  0.86 &       — &        — \\
\textbf{16 } &  3959861097024021504 &  Com Ber &                         — &   186.73234 &     23.72566 &  2.82 &       — &  18.57 &   0.25 &  1.00 &       — &        — \\
\textbf{17 } &  3959861303182454272 &  Com Ber &                         — &   186.72493 &     23.73044 &  2.78 &       — &  20.14 &   1.01 &  0.75 &       — &        — \\
\textbf{18 } &  3959861547996681728 &  Com Ber &                         — &   186.63561 &     23.71559 &  3.61 &       — &  19.81 &   0.91 &  0.77 &       — &        — \\
\textbf{19 } &  3959861960313276928 &  Com Ber &                         — &   186.63421 &     23.74742 &  3.16 &       — &  17.06 &   1.14 &  1.00 &       — &        — \\
\textbf{20 } &  3959862918090172928 &  Com Ber &                         — &   186.75199 &     23.77212 &  2.01 &       — &  20.41 &   0.75 &  0.79 &       — &        — \\
\textbf{21 } &  3959867217352720384 &  Com Ber &                         — &   186.65521 &     23.83834 &  1.73 &       — &  20.53 &   0.76 &  0.79 &       — &        — \\
\textbf{22 } &  3959870099275534336 &  Com Ber &                         — &   186.90519 &     23.89772 &  1.82 &       — &  19.70 &   0.94 &  0.94 &       — &        — \\
\textbf{23 } &  3959870167995015680 &  Com Ber &                         — &   186.88960 &     23.91535 &  1.75 &       — &  18.43 &   0.70 &  0.99 &       — &        — \\
\textbf{24 } &  3959870167995017728 &  Com Ber &                         — &   186.88796 &     23.91735 &  1.74 &       — &  19.09 &   1.00 &  0.98 &       — &        — \\
\textbf{25 } &  3959870683391090688 &  Com Ber &                         — &   186.81881 &     23.91234 &  0.91 &       — &  20.65 &   0.75 &  0.53 &       — &        — \\
\textbf{26 } &  3959871611104028672 &  Com Ber &                         — &   186.92304 &     23.91865 &  2.16 &       — &  20.17 &   0.95 &  0.69 &       — &        — \\
\textbf{27 } &  3959872027716646400 &  Com Ber &                         — &   187.00405 &     23.96026 &  3.44 &       — &  19.51 &   0.96 &  0.93 &       — &        — \\
\textbf{28 } &  3959873535249372160 &  Com Ber &                         — &   186.76510 &     23.89924 &  0.21 &       — &  19.91 &   1.00 &  0.91 &       — &        — \\
\textbf{29 } &  3959873603968850432 &  Com Ber &                         — &   186.75882 &     23.90764 &  0.18 &       — &  20.45 &   0.91 &  0.93 &       — &        — \\
\textbf{30 } &  3959873603969063936 &  Com Ber &                         — &   186.75509 &     23.91312 &  0.21 &       — &  20.67 &   0.67 &  0.95 &       — &        — \\
\textbf{31 } &  3959873947566247936 &  Com Ber &                         — &   186.76404 &     23.94180 &  0.69 &       — &  17.83 &   1.00 &  1.00 &       — &        — \\
\textbf{32 } &  3959874673415916032 &  Com Ber &                         — &   186.73706 &     23.95046 &  0.68 &       — &  20.81 &   0.78 &  0.91 &       — &        — \\
\textbf{33 } &  3959875601129415168 &  Com Ber &                         — &   186.76556 &     24.01463 &  1.81 &       — &  17.17 &   1.08 &  1.00 &       — &        — \\
\textbf{34 } &  3959875768632396800 &  Com Ber &                         — &   186.86491 &     23.98741 &  2.23 &       — &  20.23 &   0.97 &  0.78 &       — &        — \\
\textbf{35 } &  3959876077870051328 &  Com Ber &                         — &   186.83070 &     24.01264 &  2.25 &       — &  19.74 &   0.94 &  0.92 &       — &        — \\
\textbf{36 } &  3959877452259603968 &  Com Ber &                         — &   186.84851 &     24.06688 &  3.18 &       — &  18.09 &   1.04 &  0.99 &       — &        — \\
\textbf{37 } &  3959882228263617536 &  Com Ber &                         — &   186.59553 &     24.02838 &  2.02 &       — &  19.85 &   1.02 &  0.94 &       — &        — \\
\textbf{38 } &  3959884740819808256 &  Com Ber &                         — &   186.51644 &     24.00724 &  2.51 &       — &  16.85 &   1.14 &  1.00 &       — &        — \\
\textbf{39 } &  3959888486031303680 &  Com Ber &                         — &   186.68111 &     24.07936 &  2.50 &       — &  15.40 &   1.42 &  1.00 &       — &        — \\
\textbf{40 } &  3953877451666634240 &  Com Ber &                         — &   186.37624 &     23.87828 &  4.47 &       — &  18.51 &   1.06 &  0.86 &       — &        — \\
\textbf{41 } &  3959813646225316864 &  Com Ber &                         — &   186.78216 &     23.66171 &  3.59 &       — &  19.57 &   0.99 &  0.69 &       — &        — \\
\textbf{42 } &  3959816395004384768 &  Com Ber &                         — &   187.03847 &     23.65754 &  3.98 &       — &  18.35 &   0.63 &  0.91 &       — &        — \\
\textbf{43 } &                    — &     UMaI &  SDSS J103519.12+515359.5 &   158.82967 &     51.89994 &  0.85 &       — &  22.07 &   0.01 &  0.00 &   -1.41 &        g \\
\textbf{44 } &   847519608687616640 &     UMaI &                         — &   158.82316 &     51.92608 &  0.54 &  -68.31 &  18.74 &   1.28 &  0.96 &   -1.14 &      g,m \\
\textbf{45 } &   847520334538526848 &     UMaI &                         — &   158.67198 &     51.92003 &  0.28 &  -61.91 &  19.23 &   1.17 &  1.00 &   -2.20 &      g,m \\
\textbf{46 } &   847708243651375360 &     UMaI &                         — &   158.71589 &     51.97377 &  0.86 &  -64.06 &  18.59 &   1.15 &  1.00 &   -2.75 &      g,m \\
\textbf{47 } &   847708174931896832 &     UMaI &                         — &   158.67620 &     51.96635 &  0.89 &  -37.93 &  18.67 &   1.30 &  0.00 &   -2.56 &      g,m \\
\textbf{48 } &   847516172713773440 &     UMaI &                         — &   158.77871 &     51.87363 &  0.96 &  -40.00 &  18.95 &   1.17 &  0.01 &   -1.22 &        g \\
\textbf{49 } &   847706972341268608 &     UMaI &                         — &   158.47213 &     51.89850 &  1.27 &  -62.48 &  20.49 &   0.76 &  0.00 &   -1.34 &        g \\
\textbf{50 } &   847520605120030720 &     UMaI &                         — &   158.76470 &     51.93890 &  0.26 &  -68.31 &  20.44 &   0.81 &  0.99 &   -2.57 &      o,g \\
\textbf{51 } &   847706869261834112 &     UMaI &                         — &   158.62968 &     51.95030 &  0.88 &  -56.67 &  18.10 &   1.24 &  1.00 &   -2.73 &    o,g,m \\
\textbf{52 } &   849020961751785472 &     UMaI &                         — &   158.87024 &     51.95040 &  0.71 &  -57.03 &  17.82 &   1.31 &  1.00 &   -2.58 &      o,g \\
\textbf{53 } &   847706731822875648 &     UMaI &                         — &   158.59212 &     51.93622 &  0.90 &  -39.30 &  19.99 &   0.98 &  0.00 &   -1.58 &      o,g \\
\textbf{54 } &   849017590201559552 &     UMaI &                         — &   158.90282 &     51.88844 &  1.39 &  -56.53 &  20.70 &   0.51 &  0.07 &   -2.57 &      o,g \\
\textbf{55 } &   847516103994294528 &     UMaI &                         — &   158.79778 &     51.85917 &  1.26 &  -55.14 &  19.22 &   1.03 &  1.00 &   -2.30 &      o,g \\
\textbf{56 } &   847517482680353408 &     UMaI &                         — &   158.70037 &     51.84745 &  1.08 &  -56.00 &  20.45 &   0.84 &  0.83 &   -2.00 &      o,g \\
\textbf{57 } &   847519230730488960 &     UMaI &                         — &   158.71128 &     51.87782 &  0.63 &  -45.50 &  20.58 &   0.70 &  0.96 &   -1.40 &      o,g \\
\textbf{58 } &   847707556456603520 &     UMaI &                         — &   158.57182 &     51.95931 &  1.30 &  -59.07 &  19.52 &   1.10 &  0.99 &   -2.40 &      o,g \\
\textbf{59 } &   849018002518350080 &     UMaI &                         — &   158.92855 &     51.93824 &  1.06 &  -68.79 &  19.47 &   1.03 &  1.00 &   -2.00 &      o,g \\
\textbf{60 } &   847516520606648576 &     UMaI &                         — &   158.83173 &     51.88136 &  1.10 &  -58.87 &  20.48 &   0.37 &  0.99 &       — &        j \\
\textbf{61 } &   847519131947798272 &     UMaI &                         — &   158.77041 &     51.88709 &  0.72 &  -59.69 &  20.51 &   0.26 &  0.98 &       — &        j \\
\textbf{62 } &   847520025300875520 &     UMaI &                         — &   158.83978 &     51.97475 &  0.74 &  -59.86 &  20.27 &   0.68 &  0.96 &       — &        j \\
\textbf{63 } &   847520000000000000 &     UMaI &                         — &   158.72356 &     51.91511 &  0.09 &  -64.14 &  20.15 &   1.26 &  0.99 &       — &        j \\
\textbf{64 } &   847520192803168640 &     UMaI &                         — &   158.74220 &     51.92328 &  0.11 &  -51.26 &  20.01 &   0.90 &  0.99 &       — &        j \\
\textbf{65 } &   847520295882556928 &     UMaI &                         — &   158.74685 &     51.95196 &  0.43 &  -68.19 &  20.30 &   0.20 &  1.00 &       — &        j \\
\textbf{66 } &   847701371703681408 &     UMaI &                         — &   158.43684 &     51.90670 &  1.52 &  -53.51 &  20.10 &   1.10 &  0.93 &       — &        j \\
\textbf{67 } &   847706663103625984 &     UMaI &                         — &   158.62834 &     51.94127 &  0.77 &  -56.61 &  20.34 &   0.47 &  0.99 &       — &        j \\
\textbf{68 } &   847707728255299712 &     UMaI &                         — &   158.57797 &     51.97473 &  1.48 &  -73.47 &  20.11 &   0.52 &  0.83 &       — &        j \\
\textbf{69 } &   849017972454861440 &     UMaI &                         — &   158.90414 &     51.94549 &  0.89 &  -59.55 &  20.52 &   0.59 &  0.92 &       — &        j \\
\textbf{70 } &   849018002518421760 &     UMaI &                         — &   158.94180 &     51.94657 &  1.09 &  -52.63 &  20.42 &   0.28 &  0.92 &       — &        j \\
\textbf{71 } &   849018075533761408 &     UMaI &                         — &   158.93573 &     51.96584 &  1.02 &  -40.73 &  19.86 &   1.03 &  0.99 &       — &        j \\
\textbf{72 } &   849020957455855616 &     UMaI &                         — &   158.87605 &     51.95833 &  0.75 &  -52.90 &  20.33 &   0.75 &  0.98 &       — &        j \\
\textbf{73 } &   849021270989478272 &     UMaI &                         — &   158.89314 &     51.99936 &  1.07 &  -56.69 &  20.61 &   0.22 &  0.96 &       — &        j \\
\textbf{74 } &   849021507211738112 &     UMaI &                         — &   158.95634 &     52.00489 &  1.26 &  -48.74 &  19.92 &   0.84 &  0.91 &       — &        j \\
\textbf{75 } &   849022228766245120 &     UMaI &                         — &   158.90671 &     52.04344 &  1.60 &  -25.97 &  20.43 &   0.61 &  0.92 &       — &        j \\
\textbf{76 } &   847515245001014784 &     UMaI &                         — &   158.89520 &     51.82919 &  2.15 &       — &  20.48 &   0.75 &  0.86 &       — &        — \\
\textbf{77 } &   847519849205957760 &     UMaI &                         — &   158.77332 &     51.92793 &  0.26 &       — &  20.39 &   0.56 &  0.99 &       — &        — \\
\textbf{78 } &   847698932162480128 &     UMaI &                         — &   158.25768 &     51.79609 &  2.24 &       — &  20.90 &   0.55 &  0.86 &       — &        — \\
\textbf{79 } &   847700031674114560 &     UMaI &                         — &   158.43620 &     51.83499 &  1.41 &       — &  20.51 &   0.04 &  1.00 &       — &        — \\
\textbf{80 } &   847700718868881920 &     UMaI &                         — &   158.28003 &     51.83491 &  2.09 &       — &  20.43 &   0.45 &  0.84 &       — &        — \\
\textbf{81 } &   847701990178947840 &     UMaI &                         — &   158.15683 &     51.83232 &  2.72 &       — &  20.42 &   0.41 &  0.76 &       — &        — \\
\textbf{82 } &   847704326641185408 &     UMaI &                         — &   158.38426 &     51.92151 &  1.94 &       — &  20.07 &   1.08 &  0.93 &       — &        — \\
\textbf{83 } &   847704434016766720 &     UMaI &                         — &   158.39778 &     51.93318 &  1.98 &       — &  19.87 &   0.93 &  0.64 &       — &        — \\
\textbf{84 } &   847705975908854528 &     UMaI &                         — &   158.51178 &     51.87997 &  0.99 &       — &  20.54 &   0.31 &  0.98 &       — &        — \\
\textbf{85 } &   847706147707301760 &     UMaI &                         — &   158.47656 &     51.86228 &  1.16 &       — &  20.26 &   0.57 &  0.95 &       — &        — \\
\textbf{86 } &   847707006700773632 &     UMaI &                         — &   158.49136 &     51.90606 &  1.20 &       — &  20.37 &   0.54 &  0.70 &       — &        — \\
\textbf{87 } &   847707350298393472 &     UMaI &                         — &   158.47407 &     51.94437 &  1.66 &       — &  20.81 &  -0.08 &  0.73 &       — &        — \\
\textbf{88 } &   847716356845689344 &     UMaI &                         — &   158.12545 &     51.95135 &  3.72 &       — &  17.12 &   1.48 &  1.00 &       — &        — \\
\textbf{89 } &   849013638831653632 &     UMaI &                         — &   159.35696 &     52.05978 &  3.02 &       — &  20.58 &   1.02 &  0.65 &       — &        — \\
\textbf{90 } &   849017010381183744 &     UMaI &                         — &   158.98127 &     51.92640 &  1.44 &       — &  20.51 &   0.36 &  0.98 &       — &        — \\
\textbf{91 } &   849018453490931840 &     UMaI &                         — &   158.99886 &     51.97692 &  1.32 &       — &  20.58 &   0.70 &  0.74 &       — &        — \\
\textbf{92 } &   849019857944242048 &     UMaI &                         — &   159.07142 &     52.01200 &  1.69 &       — &  20.13 &   0.95 &  0.91 &       — &        — \\
\textbf{93 } &   849020167181942528 &     UMaI &                         — &   159.07563 &     52.03784 &  1.82 &       — &  20.41 &   0.47 &  0.71 &       — &        — \\
\textbf{94 } &   849020755593349376 &     UMaI &                         — &   159.18798 &     52.08359 &  2.46 &       — &  20.32 &   0.51 &  0.78 &       — &        — \\
\textbf{95 } &   849020820016978048 &     UMaI &                         — &   159.17811 &     52.10100 &  2.56 &       — &  20.42 &   0.44 &  0.89 &       — &        — \\
\textbf{96 } &   849021438492203264 &     UMaI &                         — &   158.96669 &     51.99805 &  1.24 &       — &  19.90 &   1.11 &  0.99 &       — &        — \\
\textbf{97 } &   849024363365880576 &     UMaI &                         — &   159.07709 &     52.12619 &  2.68 &       — &  20.32 &   0.71 &  0.61 &       — &        — \\
\textbf{98 } &   849024496508951680 &     UMaI &                         — &   159.02815 &     52.12170 &  2.61 &       — &  18.55 &   1.20 &  0.99 &       — &        — \\
\textbf{99 } &  1230826335841709056 &     BooI &                   Boo-007 &   209.89801 &     14.33992 &  1.19 &  114.40 &  17.60 &   1.16 &  1.00 &   -2.28 &        b \\
\textbf{100} &  1230830222787068928 &     BooI &                   Boo-033 &   210.04885 &     14.41705 &  0.48 &   98.96 &  17.49 &   1.25 &  1.00 &   -2.47 &        b \\
\textbf{101} &  1230835892143883008 &     BooI &                   Boo-094 &   210.13127 &     14.56765 &  0.78 &   95.07 &  16.60 &   1.32 &  1.00 &   -2.90 &        b \\
\textbf{102} &  1230835475531625216 &     BooI &                   Boo-117 &   210.04369 &     14.52931 &  0.20 &   99.54 &  17.44 &   1.23 &  1.00 &   -2.18 &  b,f,h,e \\
\textbf{103} &  1230861043472371456 &     BooI &                   Boo-121 &   210.15215 &     14.65759 &  1.16 &  132.74 &  17.09 &   1.29 &  1.00 &   -2.39 &        b \\
\textbf{104} &  1230837163454204672 &     BooI &                   Boo-127 &   210.06067 &     14.59797 &  0.56 &   99.00 &  17.38 &   1.27 &  1.00 &   -1.98 &        b \\
\textbf{105} &  1230649834160653312 &     BooI &                   Boo-980 &   209.80284 &     13.71547 &  4.37 &  105.00 &  17.86 &   1.08 &  0.97 &   -3.09 &      i,d \\
\textbf{106} &  1230837163454204672 &     BooI &                   Boo-127 &   210.06067 &     14.59797 &  0.56 &   99.00 &  17.38 &   1.27 &  1.00 &   -2.08 &  i,f,h,d \\
\textbf{107} &  1230744529599617280 &     BooI &                  Boo-1137 &   209.64089 &     14.35235 &  2.70 &  110.00 &  17.35 &   1.22 &  1.00 &   -3.66 &      f,d \\
\textbf{108} &  1230834826991992832 &     BooI &                   Boo-130 &   209.95406 &     14.50172 &  0.49 &  110.50 &  17.49 &   1.19 &  1.00 &   -2.29 &      f,d \\
\textbf{109} &  1230830222787068928 &     BooI &                    Boo-33 &   210.04885 &     14.41705 &  0.48 &   98.96 &  17.49 &   1.25 &  1.00 &   -2.29 &      f,d \\
\textbf{110} &  1230835892143883008 &     BooI &                   Boo-094 &   210.13127 &     14.56765 &  0.79 &   95.07 &  16.60 &   1.32 &  1.00 &   -2.90 &    f,h,d \\
\textbf{111} &  1230823247760125184 &     BooI &                   Boo-009 &   209.95335 &     14.32858 &  1.01 &  124.90 &  17.11 &   1.26 &  1.00 &   -2.67 &      h,d \\
\textbf{112} &  1230848914484728064 &     BooI &                   Boo-911 &   210.00446 &     14.61430 &  0.64 &   91.83 &  17.16 &   1.28 &  1.00 &   -1.98 &    h,d,b \\
\textbf{113} &  1230861043472371456 &     BooI &                   Boo-121 &   210.15215 &     14.65759 &  1.17 &  132.74 &  17.09 &   1.29 &  1.00 &   -2.37 &      h,d \\
\textbf{114} &  1230831047420766464 &     BooI &                    Boo-41 &   210.10763 &     14.43545 &  0.68 &  107.96 &  17.68 &   1.19 &  1.00 &   -1.93 &  f,e,o,d \\
\textbf{115} &  1230833585745988096 &     BooI &                   Boo-119 &   210.04105 &     14.47305 &  0.19 &   92.45 &  17.71 &   1.23 &  1.00 &   -3.33 &      f,o \\
\textbf{116} &  1230846676806885120 &     BooI &                    Boo08* &   209.93728 &     14.54170 &  0.66 &  101.75 &  20.33 &   0.89 &  0.84 &   -2.48 &    e,o,p \\
\textbf{117} &  1230835028855032832 &     BooI &                    Boo14* &   209.95139 &     14.53433 &  0.55 &  105.47 &  19.35 &   0.72 &  0.97 &   -2.57 &    e,o,p \\
\textbf{118} &  1230835063214777600 &     BooI &                    Boo06* &   209.96803 &     14.54602 &  0.48 &   98.55 &  20.18 &   1.02 &  0.98 &   -2.20 &    e,o,p \\
\textbf{119} &  1230833723185498112 &     BooI &                    Boo15* &   209.99103 &     14.46737 &  0.28 &  101.67 &  19.96 &   1.07 &  0.99 &   -2.89 &    e,o,p \\
\textbf{120} &  1230833963703127808 &     BooI &                    Boo07* &   210.02221 &     14.50649 &  0.04 &   98.88 &  20.60 &   0.73 &  0.92 &   -2.49 &    e,o,p \\
\textbf{121} &  1230830493370084864 &     BooI &                    Boo19* &   210.02338 &     14.43857 &  0.33 &  106.64 &  19.91 &   0.71 &  0.90 &   -3.29 &    e,o,p \\
\textbf{122} &  1230836368884839424 &     BooI &                    Boo02* &   210.05382 &     14.55327 &  0.34 &  101.25 &  18.99 &   1.06 &  1.00 &   -2.37 &    e,o,p \\
\textbf{123} &  1230830321570823424 &     BooI &                    Boo-25 &   210.09100 &     14.43150 &  0.60 &  100.35 &  20.52 &   0.86 &  0.85 &   -2.76 &    e,o,p \\
\textbf{124} &  1230835956567981824 &     BooI &                    Boo-13 &   210.09351 &     14.55748 &  0.54 &   98.30 &  19.17 &   0.80 &  0.85 &   -2.49 &    e,o,p \\
\textbf{125} &  1230835681690063872 &     BooI &                    Boo-12 &   210.11369 &     14.53877 &  0.63 &  105.29 &  19.83 &   1.03 &  0.99 &   -2.48 &    e,o,p \\
\textbf{126} &  1230832417514897920 &     BooI &                    Boo-03 &   210.13780 &     14.49991 &  0.77 &   96.62 &  19.16 &   1.01 &  1.00 &   -3.09 &    e,o,p \\
\textbf{127} &  1230830463305085184 &     BooI &                    Boo-23 &   210.04805 &     14.43224 &  0.41 &  113.29 &  21.05 &   0.61 &  0.00 &   -2.90 &      e,p \\
\textbf{128} &  1230834547819224320 &     BooI &                    Boo22* &   209.96096 &     14.48643 &  0.44 &   92.80 &  18.55 &   1.09 &  1.00 &   -2.87 &      e,o \\
\textbf{129} &  1230833963703127552 &     BooI &                         — &   210.01280 &     14.50657 &  0.09 &   97.90 &  21.04 &   0.72 &  0.00 &   -1.90 &      o,p \\
\textbf{130} &  1230833860623898624 &     BooI &                         — &   210.01386 &     14.48096 &  0.12 &  115.90 &  20.25 &   0.70 &  0.00 &   -2.32 &      o,p \\
\textbf{131} &  1230828122548139008 &     BooI &                         — &   209.91402 &     14.44401 &  0.80 &  102.01 &  19.86 &   1.05 &  0.92 &   -2.20 &      o,p \\
\textbf{132} &  1230834410380273664 &     BooI &                         — &   209.92577 &     14.49508 &  0.68 &   90.18 &  19.04 &   1.07 &  0.99 &   -2.30 &      o,p \\
\textbf{133} &  1230835578610843648 &     BooI &                   Boo-117 &   210.04369 &     14.52931 &  0.20 &   98.20 &  17.44 &   1.23 &  0.00 &   -2.25 &      o,d \\
\textbf{134} &  1230833963703127552 &     BooI &                    Boo-04 &   210.01280 &     14.50657 &  0.09 &  101.47 &  21.04 &   0.72 &  0.00 &   -2.39 &        e \\
\textbf{135} &  1230846745526363136 &     BooI &                    Boo-05 &   209.93445 &     14.54480 &  0.68 &   99.70 &  20.92 &   1.02 &  0.00 &   -2.89 &        e \\
\textbf{136} &  1230833860623898624 &     BooI &                    Boo-18 &   210.01386 &     14.48096 &  0.12 &  107.85 &  20.25 &   0.70 &  0.34 &   -2.51 &        e \\
\textbf{137} &  1230835853488763136 &     BooI &                    Boo-09 &   210.10727 &     14.55231 &  0.54 &       — &  19.52 &   0.60 &  0.07 &   -2.65 &        e \\
\textbf{138} &  1230833486962192640 &     BooI &                    Boo-28 &   210.01729 &     14.45611 &  0.29 &       — &  15.85 &   0.83 &  0.00 &   -2.31 &        e \\
\textbf{139} &  1230831803334814464 &     BooI &                    Boo-30 &   210.10087 &     14.44123 &  0.62 &       — &  20.98 &   1.64 &  0.00 &   -1.86 &        e \\
\textbf{140} &  1230724631016059904 &     BooI &                  Boo-1069 &   209.72176 &     14.11606 &  2.82 &  112.00 &  18.49 &   0.99 &  0.77 &   -2.51 &        d \\
\textbf{141} &  1230826335841709056 &     BooI &                     Boo-7 &   209.89801 &     14.33992 &  1.18 &  114.40 &  17.60 &   1.16 &  1.00 &   -2.32 &        d \\
\textbf{142} &  1230823312184726272 &     BooI &                     Boo-8 &   209.91088 &     14.32108 &  1.19 &  107.50 &  18.46 &   1.01 &  0.98 &   -2.75 &        d \\
\textbf{143} &  1230773937240652800 &     BooI &                    Boo-78 &   210.06138 &     14.22053 &  1.54 &  103.50 &  18.63 &   1.07 &  1.00 &   -2.46 &        d \\
\textbf{144} &  1230775345989954048 &     BooI &                    Boo-34 &   210.08794 &     14.29109 &  1.23 &  111.25 &  18.07 &   1.14 &  1.00 &   -3.10 &        d \\
\textbf{145} &  1231035483568837120 &     BooI &                         — &   209.42329 &     14.58663 &  4.18 &   98.70 &  19.83 &   1.02 &  0.65 &   -1.92 &        n \\
\textbf{146} &  1230843309552514304 &     BooI &                         — &   209.57916 &     14.50216 &  3.06 &  123.80 &  19.40 &   1.00 &  0.91 &   -2.43 &        n \\
\textbf{147} &  1231031497839177728 &     BooI &                         — &   209.59272 &     14.54056 &  2.99 &  106.50 &  18.87 &   1.02 &  0.92 &   -2.30 &        n \\
\textbf{148} &  1231074516231323136 &     BooI &                         — &   209.85213 &     15.04768 &  3.24 &  114.30 &  19.81 &   0.84 &  0.67 &   -2.17 &        n \\
\textbf{149} &  1230874542554264832 &     BooI &                         — &   210.05695 &     14.75375 &  1.36 &   98.20 &  19.97 &   1.02 &  0.98 &   -3.97 &        n \\
\textbf{150} &  1230887118218565632 &     BooI &                         — &   210.06789 &     14.94406 &  2.38 &  105.00 &  19.30 &   0.98 &  0.98 &   -2.56 &        n \\
\textbf{151} &  1230874954871117824 &     BooI &                         — &   210.11529 &     14.73794 &  1.38 &  114.10 &  20.05 &   0.95 &  0.98 &   -2.46 &        n \\
\textbf{152} &  1230769470474643456 &     BooI &                         — &   210.11893 &     14.12933 &  2.13 &   93.30 &  19.31 &   0.93 &  0.96 &   -2.80 &        n \\
\textbf{153} &  1230861142257868032 &     BooI &                         — &   210.16386 &     14.66974 &  1.27 &   94.80 &  20.12 &   0.99 &  0.91 &   -3.98 &        n \\
\textbf{154} &  1229998300506922496 &     BooI &                         — &   210.35767 &     13.88567 &  4.14 &  107.60 &  19.83 &   0.75 &  0.19 &   -1.90 &        n \\
\textbf{155} &  1231095269513901568 &     BooI &                         — &   210.02997 &     15.23860 &  3.96 &   96.80 &  19.78 &   0.93 &  0.75 &   -3.99 &        n \\
\textbf{156} &  1231068881234192640 &     BooI &                         — &   210.03399 &     14.92352 &  2.27 &  116.00 &  19.88 &   0.85 &  0.74 &   -2.59 &        n \\
\textbf{157} &  1230672610372100096 &     BooI &                         — &   209.99684 &     13.99147 &  2.72 &  104.40 &  19.29 &   0.96 &  0.76 &   -2.45 &        n \\
\textbf{158} &  1230849081988080896 &     BooI &                         — &   210.04421 &     14.63995 &  0.75 &  101.19 &  19.36 &   1.06 &  0.99 &   -3.00 &      k,n \\
\textbf{159} &  1230848326073809408 &     BooI &                         — &   209.98056 &     14.58134 &  0.55 &  100.03 &  19.14 &   1.10 &  1.00 &   -2.60 &    k,n,p \\
\textbf{160} &  1230847089123225856 &     BooI &                         — &   209.93098 &     14.57732 &  0.79 &   99.81 &  20.26 &   0.79 &  0.75 &   -2.28 &      k,p \\
\textbf{161} &  1230849425585454592 &     BooI &                         — &   209.93573 &     14.61934 &  0.92 &   97.93 &  19.87 &   1.04 &  0.99 &   -2.43 &      k,p \\
\textbf{162} &  1230826988676907520 &     BooI &                         — &   209.93776 &     14.39093 &  0.81 &  102.84 &  20.75 &   0.45 &  0.82 &   -1.99 &      k,p \\
\textbf{163} &  1230827297914411520 &     BooI &                         — &   209.94307 &     14.41995 &  0.68 &   98.07 &  19.89 &   0.85 &  0.55 &   -2.62 &      k,p \\
\textbf{164} &  1230848772750422272 &     BooI &                         — &   209.95056 &     14.61297 &  0.82 &  103.20 &  20.37 &   0.82 &  0.80 &   -2.14 &      k,p \\
\textbf{165} &  1230853376955406848 &     BooI &                         — &   209.95224 &     14.70124 &  1.22 &  111.75 &  19.82 &   0.86 &  0.95 &   -2.19 &      k,p \\
\textbf{166} &  1230834620833562624 &     BooI &                         — &   209.96213 &     14.50077 &  0.43 &   99.94 &  16.51 &   1.43 &  1.00 &   -2.26 &      k,p \\
\textbf{167} &  1230848600951721472 &     BooI &                         — &   209.96544 &     14.59537 &  0.68 &   99.94 &  18.83 &   1.10 &  0.98 &   -2.33 &      k,p \\
\textbf{168} &  1230833413947850752 &     BooI &                         — &   209.97132 &     14.45955 &  0.41 &  104.70 &  20.36 &   0.95 &  0.98 &   -2.56 &      k,p \\
\textbf{169} &  1230836471964048896 &     BooI &                         — &   210.00099 &     14.54305 &  0.29 &  108.27 &  20.12 &   1.01 &  0.99 &   -1.78 &      k,p \\
\textbf{170} &  1230823724501603328 &     BooI &                         — &   210.00639 &     14.36506 &  0.73 &  103.50 &  19.35 &   1.03 &  0.99 &   -2.50 &      k,p \\
\textbf{171} &  1230836643762759424 &     BooI &                         — &   210.02152 &     14.57439 &  0.40 &  104.05 &  20.46 &   0.98 &  0.97 &   -2.82 &      k,p \\
\textbf{172} &  1230848978908853248 &     BooI &                         — &   210.03612 &     14.61508 &  0.62 &  103.07 &  20.40 &   0.80 &  0.90 &   -2.32 &      k,p \\
\textbf{173} &  1230835170589373952 &     BooI &                         — &   210.04457 &     14.49012 &  0.15 &  103.55 &  19.12 &   1.05 &  1.00 &   -2.28 &      k,p \\
\textbf{174} &  1230835131934224384 &     BooI &                         — &   210.06929 &     14.49041 &  0.31 &   97.21 &  20.84 &   1.57 &  0.89 &   -2.51 &      k,p \\
\textbf{175} &  1230836059647199744 &     BooI &                         — &   210.10483 &     14.56298 &  0.62 &  100.22 &  20.52 &   0.84 &  0.94 &   -2.59 &      k,p \\
\textbf{176} &  1230832211356461056 &     BooI &                         — &   210.10625 &     14.48813 &  0.57 &  102.16 &  20.57 &   0.63 &  0.84 &   -2.42 &      k,p \\
\textbf{177} &  1230831597176581120 &     BooI &                         — &   210.15579 &     14.48278 &  0.91 &  106.95 &  16.37 &   1.47 &  1.00 &   -2.26 &      k,p \\
\textbf{178} &  1230783626686364672 &     BooI &                         — &   210.19813 &     14.40335 &  1.33 &  117.74 &  20.52 &   0.86 &  0.74 &   -2.60 &      k,p \\
\textbf{179} &  1230850009701023232 &     BooI &                         — &   209.96388 &     14.65162 &  0.94 &  111.07 &  19.57 &   0.29 &  1.00 &       — &      k,p \\
\textbf{180} &  1230848807110164736 &     BooI &                         — &   209.97871 &     14.62095 &  0.74 &  109.80 &  19.54 &   0.22 &  0.99 &       — &      k,p \\
\textbf{181} &  1230848463512766720 &     BooI &                         — &   210.00312 &     14.59139 &  0.52 &   99.52 &  19.83 &  -0.10 &  1.00 &       — &      k,p \\
\textbf{182} &  1230836953000413696 &     BooI &                         — &   210.06912 &     14.59167 &  0.56 &   99.39 &  19.62 &   0.40 &  1.00 &       — &      k,p \\
\textbf{183} &  1230860867378343680 &     BooI &                         — &   210.09209 &     14.64394 &  0.87 &   93.84 &  19.54 &   0.13 &  1.00 &       — &      k,p \\
\textbf{184} &  1230860798658865664 &     BooI &                         — &   210.11267 &     14.64176 &  0.93 &  105.37 &  19.65 &   0.23 &  1.00 &       — &      k,p \\
\textbf{185} &  1230831524161686016 &     BooI &                         — &   210.16485 &     14.47441 &  0.98 &   95.13 &  19.65 &   0.14 &  1.00 &       — &      k,p \\
\textbf{186} &  1230823174745775104 &     BooI &                         — &   209.95890 &     14.32901 &  0.99 &  102.50 &  19.74 &   0.77 &  0.11 &   -2.13 &        p \\
\textbf{187} &  1230834753977115904 &     BooI &                         — &   209.97391 &     14.51555 &  0.37 &  124.70 &  20.10 &   0.92 &  0.00 &   -0.97 &        p \\
\textbf{188} &  1230848326073804288 &     BooI &                         — &   209.98326 &     14.57381 &  0.50 &  114.80 &  19.08 &   0.95 &  0.00 &   -1.22 &        p \\
\textbf{189} &  1230830081053217792 &     BooI &                         — &   210.00688 &     14.41519 &  0.46 &   93.80 &  18.62 &   1.04 &  0.00 &   -1.27 &        p \\
\textbf{190} &  1230873649201036800 &     BooI &                         — &   210.00929 &     14.68729 &  1.02 &   80.40 &  20.30 &   0.72 &  0.00 &   -1.18 &        p \\
\textbf{191} &  1230829673030965504 &     BooI &                         — &   210.01017 &     14.38032 &  0.64 &  103.90 &  20.68 &   1.03 &  0.00 &   -2.19 &        p \\
\textbf{192} &  1230835097574485504 &     BooI &                         — &   210.05097 &     14.48945 &  0.19 &   99.20 &  20.92 &  -0.08 &  0.00 &   -2.53 &        p \\
\textbf{193} &  1230872584049134080 &     BooI &                         — &   210.06110 &     14.65854 &  0.87 &  101.00 &  20.92 &   0.22 &  0.00 &   -2.19 &        p \\
\textbf{194} &  1230832250011670784 &     BooI &                         — &   210.11075 &     14.49690 &  0.59 &  107.40 &  20.70 &   0.83 &  0.92 &   -2.38 &        p \\
\textbf{195} &  1230829256419219456 &     BooI &                         — &   210.11834 &     14.39796 &  0.87 &  100.00 &  21.00 &   0.92 &  0.00 &   -2.70 &        p \\
\textbf{196} &  1230784313881154048 &     BooI &                         — &   210.19823 &     14.44174 &  1.25 &   98.20 &  20.87 &   0.33 &  0.00 &   -2.58 &        p \\
\textbf{197} &                    — &     BooI &  SDSS J135933.50+142821.6 &   209.88958 &     14.47267 &  0.93 &  117.80 &  21.58 &   0.07 &  0.00 &   -3.14 &        p \\
\textbf{198} &                    — &     BooI &  SDSS J135937.60+142647.6 &   209.90667 &     14.44656 &  0.84 &  102.70 &  21.31 &   0.08 &  0.00 &   -2.44 &        p \\
\textbf{199} &                    — &     BooI &  SDSS J135945.72+142230.9 &   209.94050 &     14.37525 &  0.85 &   90.30 &  21.41 &   0.06 &  0.00 &   -2.02 &        p \\
\textbf{200} &                    — &     BooI &  SDSS J135947.06+142852.5 &   209.94608 &     14.48125 &  0.54 &  103.70 &  21.20 &   0.00 &  0.00 &   -2.07 &        p \\
\textbf{201} &                    — &     BooI &  SDSS J135950.75+143114.2 &   209.96146 &     14.52061 &  0.46 &   94.80 &  21.45 &   0.12 &  0.00 &   -2.04 &        p \\
\textbf{202} &                    — &     BooI &  SDSS J140000.99+143126.7 &   210.00412 &     14.52408 &  0.20 &  107.60 &  21.55 &  -0.03 &  0.00 &   -2.47 &        p \\
\textbf{203} &                    — &     BooI &  SDSS J140010.61+143823.8 &   210.04421 &     14.63994 &  0.75 &  101.10 &  19.54 &   0.22 &  0.00 &   -2.37 &        p \\
\textbf{204} &                    — &     BooI &  SDSS J140015.80+143446.8 &   210.06588 &     14.57967 &  0.49 &  118.60 &  21.53 &  -0.03 &  0.00 &   -2.93 &        p \\
\textbf{205} &                    — &     BooI &  SDSS J140023.33+142607.9 &   210.09721 &     14.43556 &  0.62 &   93.40 &  21.53 &   0.10 &  0.00 &   -1.11 &        p \\
\textbf{206} &                    — &     BooI &  SDSS J140028.93+142502.2 &   210.12058 &     14.41728 &  0.82 &  101.30 &  21.54 &   0.05 &  0.00 &   -2.33 &        p \\
\textbf{207} &                    — &     BooI &  SDSS J140057.91+142854.0 &   210.24133 &     14.48167 &  1.49 &   98.50 &  21.34 &  -0.02 &  0.00 &   -2.05 &        p \\
\textbf{208} &  1230849361161115904 &     BooI &                         — &   210.01448 &     14.66452 &  0.89 &  105.50 &  21.38 &   1.07 &  0.00 &       — &        p \\
\textbf{209} &                    — &     BooI &  SDSS J135934.37+143017.1 &   209.89321 &     14.50475 &  0.91 &   77.90 &  21.62 &   0.09 &  0.00 &       — &        p \\
\textbf{210} &                    — &     BooI &  SDSS J135945.70+142552.5 &   209.94046 &     14.43125 &  0.66 &   99.00 &  22.03 &   0.09 &  0.00 &       — &        p \\
\textbf{211} &                    — &     BooI &  SDSS J135951.07+143049.8 &   209.96283 &     14.51383 &  0.44 &  104.80 &  21.68 &   0.03 &  0.00 &       — &        p \\
\textbf{212} &                    — &     BooI &  SDSS J135953.00+142232.1 &   209.97088 &     14.37558 &  0.74 &  102.30 &  21.93 &  -0.06 &  0.00 &       — &        p \\
\textbf{213} &                    — &     BooI &  SDSS J140002.28+142653.4 &   210.00954 &     14.44817 &  0.29 &  108.70 &  21.47 &   0.11 &  0.00 &       — &        p \\
\textbf{214} &                    — &     BooI &  SDSS J140010.30+142626.5 &   210.04296 &     14.44072 &  0.35 &  102.10 &  21.70 &   0.09 &  0.00 &       — &        p \\
\textbf{215} &                    — &     BooI &  SDSS J140020.58+143734.0 &   210.08579 &     14.62611 &  0.77 &  104.40 &  21.87 &   0.02 &  0.00 &       — &        p \\
\textbf{216} &                    — &     BooI &  SDSS J140023.37+143245.2 &   210.09742 &     14.54589 &  0.54 &   97.40 &  21.28 &  -0.06 &  0.00 &       — &        p \\
\textbf{217} &  1230834925776358656 &     BooI &                         — &   209.94143 &     14.52796 &  0.60 &  131.30 &  19.46 &   0.51 &  0.99 &       — &        l \\
\textbf{218} &  1230841110529260032 &     BooI &                         — &   209.75971 &     14.50644 &  1.82 &   92.14 &  17.64 &   1.16 &  1.00 &       — &        l \\
\textbf{219} &  1230819841851105536 &     BooI &                         — &   209.90330 &     14.19465 &  1.78 &   91.00 &  19.08 &   1.12 &  0.99 &       — &        l \\
\textbf{220} &  1230774624435416832 &     BooI &                         — &   210.01257 &     14.21000 &  1.55 &   95.00 &  19.48 &   0.92 &  0.96 &       — &        l \\
\textbf{221} &  1230767271451373824 &     BooI &                         — &   210.02437 &     14.05914 &  2.36 &   95.30 &  18.32 &   1.13 &  0.99 &       — &        l \\
\textbf{222} &  1230775449069163520 &     BooI &                         — &   210.02693 &     14.27514 &  1.21 &  114.00 &  19.34 &   0.95 &  0.94 &       — &        l \\
\textbf{223} &  1229895702327886336 &     BooI &                         — &   210.07118 &     13.65910 &  4.54 &   98.00 &  18.71 &   1.12 &  0.93 &       — &        l \\
\textbf{224} &  1230873275539233536 &     BooI &                         — &   210.13332 &     14.71734 &  1.34 &  105.03 &  17.46 &   1.26 &  1.00 &       — &        l \\
\textbf{225} &  1230713292302089728 &     BooI &                         — &   209.15700 &     14.10564 &  6.18 &       — &  19.43 &   0.33 &  0.75 &       — &        — \\
\textbf{226} &  1230745590456548096 &     BooI &                         — &   209.48188 &     14.31368 &  3.79 &       — &  19.69 &   0.12 &  0.99 &       — &        — \\
\textbf{227} &  1230744456585187328 &     BooI &                         — &   209.61219 &     14.33958 &  2.90 &       — &  20.64 &   1.18 &  0.52 &       — &        — \\
\textbf{228} &  1231064517547444736 &     BooI &                         — &   209.61268 &     15.01416 &  4.08 &       — &  19.52 &   0.45 &  0.90 &       — &        — \\
\textbf{229} &  1230717346751479808 &     BooI &                         — &   209.67074 &     14.03534 &  3.36 &       — &  18.70 &   1.08 &  0.97 &       — &        — \\
\textbf{230} &  1231039885910013440 &     BooI &                         — &   209.67834 &     14.66212 &  2.59 &       — &  19.29 &   0.99 &  0.96 &       — &        — \\
\textbf{231} &  1230731468604067328 &     BooI &                         — &   209.68330 &     14.27127 &  2.57 &       — &  20.61 &   1.03 &  0.69 &       — &        — \\
\textbf{232} &  1231547855987547392 &     BooI &                         — &   209.68346 &     15.73852 &  7.19 &       — &  19.67 &   0.22 &  0.65 &       — &        — \\
\textbf{233} &  1231048127952212224 &     BooI &                         — &   209.68586 &     14.88807 &  3.22 &       — &  19.76 &   0.55 &  0.76 &       — &        — \\
\textbf{234} &  1230668281045015808 &     BooI &                         — &   209.69574 &     13.90590 &  3.77 &       — &  19.72 &   0.19 &  0.98 &       — &        — \\
\textbf{235} &  1230837949433295872 &     BooI &                         — &   209.74540 &     14.38947 &  1.97 &       — &  20.56 &   0.86 &  0.63 &       — &        — \\
\textbf{236} &  1230852483602707456 &     BooI &                         — &   209.75847 &     14.67250 &  2.10 &       — &  20.16 &   0.99 &  0.84 &       — &        — \\
\textbf{237} &  1230825339409289728 &     BooI &                         — &   209.77648 &     14.31665 &  1.91 &       — &  19.39 &   0.52 &  0.84 &       — &        — \\
\textbf{238} &  1230826060963809792 &     BooI &                         — &   209.77952 &     14.35699 &  1.80 &       — &  20.36 &   0.80 &  0.79 &       — &        — \\
\textbf{239} &  1230850971774212608 &     BooI &                         — &   209.78081 &     14.61713 &  1.83 &       — &  19.68 &   0.05 &  1.00 &       — &        — \\
\textbf{240} &  1231097197954353920 &     BooI &                         — &   209.78656 &     15.21846 &  4.29 &       — &  19.65 &   0.92 &  0.72 &       — &        — \\
\textbf{241} &  1230839495621857024 &     BooI &                         — &   209.78757 &     14.40695 &  1.67 &       — &  20.06 &   0.91 &  0.87 &       — &        — \\
\textbf{242} &  1230668693361894144 &     BooI &                         — &   209.79164 &     13.93685 &  3.32 &       — &  19.52 &   0.44 &  0.69 &       — &        — \\
\textbf{243} &  1231042321156413696 &     BooI &                         — &   209.79239 &     14.77654 &  2.25 &       — &  20.55 &   0.97 &  0.76 &       — &        — \\
\textbf{244} &  1230841144888992256 &     BooI &                         — &   209.79748 &     14.48898 &  1.56 &       — &  19.69 &   0.10 &  1.00 &       — &        — \\
\textbf{245} &  1231073970770833664 &     BooI &                         — &   209.81997 &     15.00991 &  3.16 &       — &  20.94 &   0.73 &  0.63 &       — &        — \\
\textbf{246} &  1231067163247259904 &     BooI &                         — &   209.82685 &     14.84828 &  2.38 &       — &  19.52 &   0.33 &  0.99 &       — &        — \\
\textbf{247} &  1230851246652121344 &     BooI &                         — &   209.84872 &     14.62471 &  1.42 &       — &  19.17 &   1.13 &  0.95 &       — &        — \\
\textbf{248} &  1230678314088732672 &     BooI &                         — &   209.84955 &     14.10324 &  2.37 &       — &  20.20 &   0.76 &  0.58 &       — &        — \\
\textbf{249} &  1230827542727194624 &     BooI &                         — &   209.85214 &     14.38899 &  1.29 &       — &  20.64 &   0.72 &  0.80 &       — &        — \\
\textbf{250} &  1230651925809484800 &     BooI &                         — &   209.85708 &     13.80260 &  3.83 &       — &  19.72 &   0.12 &  0.98 &       — &        — \\
\textbf{251} &  1230827538432572416 &     BooI &                         — &   209.85726 &     14.39589 &  1.24 &       — &  19.44 &   0.67 &  0.97 &       — &        — \\
\textbf{252} &  1230826679439105024 &     BooI &                         — &   209.85783 &     14.37071 &  1.30 &       — &  20.57 &   0.88 &  0.78 &       — &        — \\
\textbf{253} &  1230848016836700416 &     BooI &                         — &   209.86137 &     14.58644 &  1.24 &       — &  20.82 &   0.68 &  0.89 &       — &        — \\
\textbf{254} &  1231073829036540160 &     BooI &                         — &   209.86327 &     15.00787 &  3.01 &       — &  19.70 &   0.42 &  0.87 &       — &        — \\
\textbf{255} &  1230847364001656832 &     BooI &                         — &   209.86582 &     14.55203 &  1.15 &       — &  19.74 &   0.03 &  1.00 &       — &        — \\
\textbf{256} &  1230819704412148224 &     BooI &                         — &   209.87232 &     14.17873 &  1.95 &       — &  19.50 &   0.26 &  1.00 &       — &        — \\
\textbf{257} &  1231098980365655296 &     BooI &                         — &   209.87641 &     15.26266 &  4.28 &       — &  19.49 &   0.88 &  0.86 &       — &        — \\
\textbf{258} &  1231067678643343104 &     BooI &                         — &   209.89229 &     14.88711 &  2.32 &       — &  19.66 &   0.97 &  0.95 &       — &        — \\
\textbf{259} &  1231099014725393408 &     BooI &                         — &   209.89410 &     15.26219 &  4.24 &       — &  19.58 &   0.12 &  0.99 &       — &        — \\
\textbf{260} &  1230846539367928832 &     BooI &                         — &   209.89438 &     14.53361 &  0.93 &       — &  19.67 &   0.11 &  0.99 &       — &        — \\
\textbf{261} &  1230828156907873792 &     BooI &                         — &   209.89486 &     14.43174 &  0.94 &       — &  19.62 &   0.12 &  0.99 &       — &        — \\
\textbf{262} &  1230820151088760832 &     BooI &                         — &   209.89824 &     14.22768 &  1.65 &       — &  19.46 &   1.04 &  0.95 &       — &        — \\
\textbf{263} &  1230826542000661504 &     BooI &                         — &   209.90507 &     14.36265 &  1.06 &       — &  19.86 &   0.84 &  0.91 &       — &        — \\
\textbf{264} &  1230878253406017024 &     BooI &                         — &   209.91093 &     14.77480 &  1.72 &       — &  20.87 &   1.07 &  0.82 &       — &        — \\
\textbf{265} &  1230853553049414400 &     BooI &                         — &   209.91204 &     14.71430 &  1.43 &       — &  18.98 &   1.08 &  0.99 &       — &        — \\
\textbf{266} &  1230823312184727808 &     BooI &                         — &   209.91798 &     14.32722 &  1.14 &       — &  20.86 &   0.47 &  0.68 &       — &        — \\
\textbf{267} &  1230827160475452928 &     BooI &                         — &   209.91876 &     14.40405 &  0.86 &       — &  20.32 &   1.15 &  0.92 &       — &        — \\
\textbf{268} &  1231066647851184896 &     BooI &                         — &   209.92313 &     14.84950 &  2.04 &       — &  18.62 &   1.08 &  0.99 &       — &        — \\
\textbf{269} &  1230651341693932544 &     BooI &                         — &   209.92565 &     13.80315 &  3.75 &       — &  19.52 &   0.22 &  0.99 &       — &        — \\
\textbf{270} &  1230846745526362624 &     BooI &                         — &   209.92794 &     14.54405 &  0.72 &       — &  18.79 &   0.88 &  0.97 &       — &        — \\
\textbf{271} &  1230849837902330368 &     BooI &                         — &   209.94273 &     14.64852 &  1.01 &       — &  19.59 &   0.23 &  1.00 &       — &        — \\
\textbf{272} &  1230834135502357504 &     BooI &                         — &   209.94697 &     14.46561 &  0.55 &       — &  19.58 &   0.54 &  0.96 &       — &        — \\
\textbf{273} &  1230833276508895744 &     BooI &                         — &   209.94754 &     14.44997 &  0.58 &       — &  19.96 &   0.87 &  0.72 &       — &        — \\
\textbf{274} &  1230878837521588736 &     BooI &                         — &   209.95242 &     14.82159 &  1.83 &       — &  20.47 &   0.83 &  0.67 &       — &        — \\
\textbf{275} &  1230772597210842624 &     BooI &                         — &   209.95568 &     14.16816 &  1.81 &       — &  19.43 &   0.51 &  0.95 &       — &        — \\
\textbf{276} &  1230846814245300736 &     BooI &                         — &   209.95721 &     14.54836 &  0.55 &       — &  20.70 &   0.62 &  0.74 &       — &        — \\
\textbf{277} &  1230848704030941184 &     BooI &                         — &   209.96416 &     14.60385 &  0.72 &       — &  18.81 &   0.96 &  1.00 &       — &        — \\
\textbf{278} &  1230848708325982208 &     BooI &                         — &   209.96553 &     14.59984 &  0.70 &       — &  20.63 &   0.64 &  0.91 &       — &        — \\
\textbf{279} &  1230877772369686272 &     BooI &                         — &   209.97579 &     14.78907 &  1.61 &       — &  19.54 &   1.08 &  0.92 &       — &        — \\
\textbf{280} &  1230836540683527936 &     BooI &                         — &   209.98028 &     14.54639 &  0.41 &       — &  19.53 &   0.40 &  1.00 &       — &        — \\
\textbf{281} &  1230848326073809408 &     BooI &                         — &   209.98331 &     14.58193 &  0.54 &       — &  19.58 &   0.54 &  0.72 &       — &        — \\
\textbf{282} &  1230834994495293952 &     BooI &                         — &   209.98427 &     14.53382 &  0.34 &       — &  20.22 &   0.94 &  0.96 &       — &        — \\
\textbf{283} &  1231068434557592832 &     BooI &                         — &   209.99120 &     14.91901 &  2.27 &       — &  19.65 &   0.22 &  0.99 &       — &        — \\
\textbf{284} &  1230822040874388224 &     BooI &                         — &   209.99145 &     14.26899 &  1.24 &       — &  20.70 &   0.61 &  0.51 &       — &        — \\
\textbf{285} &  1230833517027065600 &     BooI &                         — &   209.99869 &     14.45941 &  0.27 &       — &  19.41 &   0.60 &  0.94 &       — &        — \\
\textbf{286} &  1230829668736347904 &     BooI &                         — &   210.00170 &     14.38738 &  0.61 &       — &  19.16 &   1.04 &  1.00 &       — &        — \\
\textbf{287} &  1230878700082638336 &     BooI &                         — &   210.00525 &     14.83133 &  1.79 &       — &  20.31 &   0.93 &  0.91 &       — &        — \\
\textbf{288} &  1230877531851510272 &     BooI &                         — &   210.00957 &     14.77154 &  1.47 &       — &  19.12 &   1.00 &  0.99 &       — &        — \\
\textbf{289} &  1230833860623901696 &     BooI &                         — &   210.01187 &     14.48568 &  0.11 &       — &  20.90 &  -0.21 &  0.98 &       — &        — \\
\textbf{290} &  1230830012333739008 &     BooI &                         — &   210.01649 &     14.40727 &  0.50 &       — &  19.60 &   0.21 &  1.00 &       — &        — \\
\textbf{291} &  1230873614841298944 &     BooI &                         — &   210.01965 &     14.68868 &  1.01 &       — &  20.62 &   0.47 &  0.68 &       — &        — \\
\textbf{292} &  1230830497665159680 &     BooI &                         — &   210.02163 &     14.44077 &  0.32 &       — &  19.65 &  -0.07 &  1.00 &       — &        — \\
\textbf{293} &  1230833482666763264 &     BooI &                         — &   210.02354 &     14.45130 &  0.26 &       — &  19.38 &   0.66 &  0.98 &       — &        — \\
\textbf{294} &  1230873786640002304 &     BooI &                         — &   210.02541 &     14.71379 &  1.15 &       — &  19.61 &   0.53 &  0.99 &       — &        — \\
\textbf{295} &  1231068778154976256 &     BooI &                         — &   210.02653 &     14.91695 &  2.23 &       — &  19.42 &   1.02 &  0.79 &       — &        — \\
\textbf{296} &  1230835441171882496 &     BooI &                         — &   210.02657 &     14.51549 &  0.08 &       — &  20.65 &   0.85 &  0.91 &       — &        — \\
\textbf{297} &  1230836437604328704 &     BooI &                         — &   210.03704 &     14.57336 &  0.40 &       — &  19.52 &   0.55 &  0.98 &       — &        — \\
\textbf{298} &  1230877566211251712 &     BooI &                         — &   210.04219 &     14.77930 &  1.49 &       — &  19.14 &   1.03 &  1.00 &       — &        — \\
\textbf{299} &  1230775483428906496 &     BooI &                         — &   210.04608 &     14.28973 &  1.15 &       — &  20.39 &   0.66 &  0.50 &       — &        — \\
\textbf{300} &  1230772047455028224 &     BooI &                         — &   210.04614 &     14.16752 &  1.80 &       — &  20.53 &   0.98 &  0.52 &       — &        — \\
\textbf{301} &  1230829771815569664 &     BooI &                         — &   210.04618 &     14.40544 &  0.54 &       — &  19.37 &   0.64 &  0.96 &       — &        — \\
\textbf{302} &  1230659588031211264 &     BooI &                         — &   210.05592 &     13.91323 &  3.17 &       — &  19.01 &   0.98 &  0.90 &       — &        — \\
\textbf{303} &  1230879181118967808 &     BooI &                         — &   210.05699 &     14.80942 &  1.66 &       — &  20.63 &   0.58 &  0.62 &       — &        — \\
\textbf{304} &  1230874164597130496 &     BooI &                         — &   210.06166 &     14.72849 &  1.23 &       — &  19.44 &   1.01 &  0.99 &       — &        — \\
\textbf{305} &  1230829393857871616 &     BooI &                         — &   210.06497 &     14.40355 &  0.60 &       — &  19.63 &   0.20 &  1.00 &       — &        — \\
\textbf{306} &  1230830184131867392 &     BooI &                         — &   210.06672 &     14.42473 &  0.51 &       — &  19.15 &   1.07 &  1.00 &       — &        — \\
\textbf{307} &  1230835544251105280 &     BooI &                         — &   210.06731 &     14.52972 &  0.32 &       — &  20.66 &   0.71 &  0.87 &       — &        — \\
\textbf{308} &  1230828947181261824 &     BooI &                         — &   210.07734 &     14.38042 &  0.76 &       — &  18.90 &   1.13 &  1.00 &       — &        — \\
\textbf{309} &  1230661065502765824 &     BooI &                         — &   210.08096 &     13.99395 &  2.77 &       — &  18.12 &   1.13 &  0.99 &       — &        — \\
\textbf{310} &  1230873412977867520 &     BooI &                         — &   210.08316 &     14.72135 &  1.22 &       — &  20.51 &   0.66 &  0.85 &       — &        — \\
\textbf{311} &  1230829118979954432 &     BooI &                         — &   210.08941 &     14.38281 &  0.79 &       — &  19.86 &   1.01 &  0.99 &       — &        — \\
\textbf{312} &  1230860695583613696 &     BooI &                         — &   210.08976 &     14.62465 &  0.78 &       — &  19.52 &   0.56 &  1.00 &       — &        — \\
\textbf{313} &  1231078398881778432 &     BooI &                         — &   210.09065 &     15.08788 &  3.15 &       — &  19.81 &  -0.16 &  0.64 &       — &        — \\
\textbf{314} &  1230887083858828032 &     BooI &                         — &   210.09103 &     14.94891 &  2.42 &       — &  20.09 &   1.09 &  0.85 &       — &        — \\
\textbf{315} &  1230829153339697664 &     BooI &                         — &   210.10535 &     14.39135 &  0.83 &       — &  20.37 &   1.06 &  0.96 &       — &        — \\
\textbf{316} &  1230835853488763136 &     BooI &                         — &   210.10727 &     14.55231 &  0.61 &       — &  19.52 &   0.60 &  1.00 &       — &        — \\
\textbf{317} &  1230859630427736832 &     BooI &                         — &   210.11190 &     14.59251 &  0.75 &       — &  19.46 &   0.32 &  1.00 &       — &        — \\
\textbf{318} &  1230861210975733504 &     BooI &                         — &   210.12488 &     14.65789 &  1.05 &       — &  19.87 &   1.00 &  0.97 &       — &        — \\
\textbf{319} &  1230835784769285632 &     BooI &                         — &   210.12736 &     14.55158 &  0.74 &       — &  19.51 &   0.32 &  0.99 &       — &        — \\
\textbf{320} &  1230874748712681984 &     BooI &                         — &   210.13725 &     14.72687 &  1.39 &       — &  19.59 &   0.37 &  0.96 &       — &        — \\
\textbf{321} &  1230780637390847232 &     BooI &                         — &   210.15527 &     14.31491 &  1.38 &       — &  20.80 &   0.54 &  0.78 &       — &        — \\
\textbf{322} &  1230777201415813632 &     BooI &                         — &   210.16811 &     14.25687 &  1.69 &       — &  20.54 &   0.80 &  0.53 &       — &        — \\
\textbf{323} &  1230860111464091648 &     BooI &                         — &   210.16937 &     14.62892 &  1.17 &       — &  19.63 &   0.07 &  1.00 &       — &        — \\
\textbf{324} &  1230859909601056768 &     BooI &                         — &   210.17197 &     14.61236 &  1.14 &       — &  20.10 &   0.89 &  0.96 &       — &        — \\
\textbf{325} &  1229890376568407296 &     BooI &                         — &   210.17969 &     13.55215 &  5.26 &       — &  19.68 &   0.17 &  0.86 &       — &        — \\
\textbf{326} &  1230875538986689536 &     BooI &                         — &   210.18061 &     14.78411 &  1.80 &       — &  20.56 &   0.78 &  0.79 &       — &        — \\
\textbf{327} &  1230783729765579520 &     BooI &                         — &   210.18768 &     14.40273 &  1.26 &       — &  20.74 &   0.74 &  0.74 &       — &        — \\
\textbf{328} &  1231459963776551936 &     BooI &                         — &   210.19247 &     15.28623 &  4.29 &       — &  19.64 &   0.20 &  0.97 &       — &        — \\
\textbf{329} &  1230777270134712064 &     BooI &                         — &   210.19585 &     14.26598 &  1.78 &       — &  20.64 &   0.62 &  0.69 &       — &        — \\
\textbf{330} &  1230875435907473920 &     BooI &                         — &   210.19759 &     14.78402 &  1.86 &       — &  20.39 &   1.16 &  0.64 &       — &        — \\
\textbf{331} &  1230855163661700608 &     BooI &                         — &   210.20173 &     14.50640 &  1.21 &       — &  20.17 &   0.88 &  0.92 &       — &        — \\
\textbf{332} &  1230769882791510528 &     BooI &                         — &   210.20489 &     14.16427 &  2.25 &       — &  20.77 &   1.01 &  0.65 &       — &        — \\
\textbf{333} &  1230875474562491904 &     BooI &                         — &   210.21257 &     14.79886 &  1.98 &       — &  19.68 &   0.17 &  0.98 &       — &        — \\
\textbf{334} &  1230863513078248704 &     BooI &                         — &   210.21792 &     14.75422 &  1.83 &       — &  19.21 &   0.88 &  0.93 &       — &        — \\
\textbf{335} &  1230784039003230720 &     BooI &                         — &   210.22499 &     14.41309 &  1.48 &       — &  20.65 &   0.70 &  0.52 &       — &        — \\
\textbf{336} &  1230881792459098624 &     BooI &                         — &   210.23772 &     14.85467 &  2.31 &       — &  19.69 &   0.95 &  0.72 &       — &        — \\
\textbf{337} &  1230856572411010304 &     BooI &                         — &   210.24859 &     14.57166 &  1.55 &       — &  19.84 &   0.72 &  0.75 &       — &        — \\
\textbf{338} &  1230756791731180032 &     BooI &                         — &   210.27146 &     14.09729 &  2.83 &       — &  20.78 &   0.83 &  0.60 &       — &        — \\
\textbf{339} &  1230776376781505536 &     BooI &                         — &   210.27720 &     14.24164 &  2.29 &       — &  19.46 &   0.63 &  0.51 &       — &        — \\
\textbf{340} &  1230779473453197056 &     BooI &                         — &   210.28911 &     14.34780 &  2.04 &       — &  20.42 &   0.91 &  0.55 &       — &        — \\
\textbf{341} &  1230882273495441408 &     BooI &                         — &   210.29304 &     14.87886 &  2.64 &       — &  19.59 &   0.27 &  0.94 &       — &        — \\
\textbf{342} &  1231265251434486016 &     BooI &                         — &   210.29471 &     15.10058 &  3.60 &       — &  16.31 &   1.44 &  1.00 &       — &        — \\
\textbf{343} &  1230753561915765760 &     BooI &                         — &   210.30546 &     14.06466 &  3.13 &       — &  20.80 &   0.96 &  0.56 &       — &        — \\
\textbf{344} &  1230857465764224256 &     BooI &                         — &   210.30977 &     14.60247 &  1.99 &       — &  19.64 &   0.15 &  1.00 &       — &        — \\
\textbf{345} &  1230751534691179520 &     BooI &                         — &   210.31906 &     13.94736 &  3.70 &       — &  20.08 &   1.00 &  0.62 &       — &        — \\
\textbf{346} &  1230764179074370304 &     BooI &                         — &   210.32553 &     14.18046 &  2.77 &       — &  19.99 &   0.99 &  0.76 &       — &        — \\
\textbf{347} &  1230751981367787008 &     BooI &                         — &   210.32660 &     13.99796 &  3.51 &       — &  19.72 &   1.14 &  0.86 &       — &        — \\
\textbf{348} &  1230763423160123392 &     BooI &                         — &   210.32679 &     14.16674 &  2.83 &       — &  18.19 &   1.08 &  0.98 &       — &        — \\
\textbf{349} &  1230857190886308352 &     BooI &                         — &   210.33151 &     14.58303 &  2.12 &       — &  19.84 &   0.88 &  0.80 &       — &        — \\
\textbf{350} &  1230884335079756288 &     BooI &                         — &   210.34918 &     14.93722 &  3.11 &       — &  20.96 &   0.44 &  0.74 &       — &        — \\
\textbf{351} &  1230884472518714368 &     BooI &                         — &   210.37436 &     14.96069 &  3.31 &       — &  19.73 &   1.13 &  0.82 &       — &        — \\
\textbf{352} &  1230864990546977792 &     BooI &                         — &   210.37687 &     14.70699 &  2.58 &       — &  19.83 &   1.01 &  0.79 &       — &        — \\
\textbf{353} &  1231264907837100800 &     BooI &                         — &   210.38561 &     15.11408 &  3.97 &       — &  16.52 &   1.41 &  1.00 &       — &        — \\
\textbf{354} &  1230809774447356928 &     BooI &                         — &   210.45113 &     14.57703 &  2.92 &       — &  19.57 &   0.64 &  0.64 &       — &        — \\
\textbf{355} &  1230789197259464192 &     BooI &                         — &   210.47068 &     14.27833 &  3.36 &       — &  20.04 &   1.04 &  0.67 &       — &        — \\
\textbf{356} &  1230805651278706432 &     BooI &                         — &   210.47713 &     14.49475 &  3.10 &       — &  19.13 &   1.17 &  0.62 &       — &        — \\
\textbf{357} &  1231271431892634624 &     BooI &                         — &   210.69886 &     15.25604 &  5.92 &       — &  19.49 &   1.01 &  0.57 &       — &        — \\
\textbf{358} &  1231258478271048192 &     BooI &                         — &   210.70010 &     15.15507 &  5.60 &       — &  19.65 &   0.30 &  0.81 &       — &        — \\
\textbf{359} &  1229802209479252992 &     BooI &                         — &   210.72214 &     13.08108 &  9.28 &       — &  19.64 &   0.02 &  0.61 &       — &        — \\
\bottomrule
% \label{tab:allgalstars}

\end{longtable}


 

\end{landscape}
